Mining Open Semantics from CLIP: A Relation Transition Perspective for Few-Shot Learning

Contrastive Vision-Language Pre-training(CLIP) demonstrates impressive zero-shot capability. The key to improve the adaptation of CLIP to downstream task with few exemplars lies in how to effectively model and transfer the useful knowledge embedded in CLIP. Previous work mines the knowledge typically based on the limited visual samples and close-set semantics (i.e., within target category set of downstream task). However, the aligned CLIP image/text encoders contain abundant relationships between visual features and almost infinite open semantics, which may benefit the few-shot learning but remains unexplored. In this paper, we propose to mine open semantics as anchors to perform a relation transition from image-anchor relationship to image-target relationship to make predictions. Specifically, we adopt a transformer module which takes the visual feature as "Query", the text features of the anchors as "Key" and the similarity matrix between the text features of anchor and target classes as "Value". In this way, the output of such a transformer module represents the relationship between the image and target categories, i.e., the classification predictions. To avoid manually selecting the open semantics, we make the [CLASS] token of input text embedding learnable. We conduct extensive experiments on eleven representative classification datasets. The results show that our method performs favorably against previous state-of-the-arts considering few-shot classification settings.

==> rebuttal/0-OfficialComment.tex <==
Our method approaches image classification from the standpoint of relation transitions, with the goal of enhancing prediction performance through open semantic relation transitions. 
Initially, we delve into the zero-shot setting to explore which anchor patterns are advantageous for facilitating relation transitions and subsequently improving prediction performance.
The objective of the zero-shot setting is not to attain state-of-the-art performance, but rather to offer intuitive and theoretical insights into image classification within a few-shot setting.


\subsection{Method}

Our method approaches image classification from the standpoint of relation transitions, with the goal of enhancing prediction performance through open semantic relation transitions. 
Initially, we delve into the zero-shot setting to explore which anchor patterns are advantageous for facilitating relation transitions and subsequently improving prediction performance.
The objective of the zero-shot setting is not to attain state-of-the-art performance, but rather to offer intuitive and theoretical insights into image classification within a few-shot setting.
Furthermore, deriving performance improvements from the zero-shot setting, the performance enhancement brought to Caltech101 by utilizing the DTD dataset with only 47 categories significantly outweighs the performance improvement from ImageNet with its 1000 categories. 
This suggests that the pattern of the anchors appears to hold greater significance relative to their quantity.

We carry out zero-shot experiments by utilizing category names from various datasets as anchors for the Caltech101 dataset.
Through this, we identified two crucial conditions that anchors, which enhance model performance, may fulfill. 
Given the impracticality of manually selecting anchors in a zero-shot scenario, we transitioned to allowing the model to autonomously learn anchors in a few-shot environment. 
Furthermore, we employed a Transformer to replace the conventional formula-based relation transition method, enabling the model to independently acquire the skill of performing relation transitions.
As illustrated in Figure 4, the learned anchors do, to a certain degree, exhibit the two patterns that we identified as beneficial for enhancing model performance in the zero-shot setting.

\review{\nr}{About open-word semantics.}
Given that anchors undergo random initialization and are subject to training, they are expected to exhibit characteristics aligned with the open-world concept. Additionally, drawing from the "a photo of \{cls\}" learning mechanism, it is reasonable to assume that the acquired anchors are semantic nouns. 
Drawing inspiration from CoOp, we search within the lexicon, identifying a set of words that closely resemble the learned anchors. A subset of these anchors appears to align with specific semantic elements. Nevertheless, as noted by CoOp, the veracity of any deductions derived from this method remains uncertain, as the anchors learned by the model might encapsulate meanings that extend beyond the confines of the current vocabulary.

\review{\nr~\nrr}{Difference with prompt learning methods.}
While CoOp's methodology is designed to acquire contextual information, our approach is centered around learning suitable categories to serve as anchors. 
Additionally, we expanded our research by conducting experiments that involve making context information a learnable prompt, encompassing both unified and class-specific configurations, which can be found in Tab.~R4~(supplementary PDF).

\review{\nrr}{Difference with methods based on autocorrelation matrix}
In previous covariance-based few-shot learning methods, such as CovaMNet, the features are obtained from the support set. These support image features, which play a pivotal role in classification, align with the features of target categories. If measured using CLIP, the similarity distribution between any support set's image features and the target categories should exhibit an unimodal distribution. Methods of this nature rely on features that align with the target categories.

As discussed in the "Effect of different choices of anchors" subsection, we anticipate that anchors beneficial for enhancing model performance should not adhere to an unimodal similarity distribution with target categories. Instead, we seek to learn diverse anchors, and the associated similarity distribution should not be uniformly distributed.

From our perspective, the zero-shot branch of CLIP appears to be more conceptually aligned with previous methods, as the features learned from text categories in CLIP can be viewed as an expectation of the support set image features in prior methods. In contrast, our approach aims to enhance CLIP's classification performance by learning features distinct from target categories through relation transition. Furthermore, based on our understanding, the relation transition in covariance-based methods seems to differ from our approach's relation transition. 

Additionally, our methodology is rooted in CLIP. Our objective revolves around exploring the open semantics constructed by CLIP to enhance model predictions. Thus, from a macro perspective, our starting point diverges from previous approaches that rely on support image sets.

\review{\nrr}{More broader tasks.}
The methodology based on relation transitions can equally be extended to semantic segmentation tasks. We performed brief experiments on the VOC dataset as a quick showcase of the efficacy of our approach, which can be found in Tab.~R4~(supplementary PDF).

\subsection{Anchors}

\review{\nr~\nrrr~\nrrrr}{Selection of anchors in zero-shot setting.}
We chose the remaining ten datasets from the pool of eleven datasets, excluding the dataset used for testing, to serve as anchors~(ten groups). Among these, we selected the group of anchors that demonstrated the highest performance and reported it in Table 1.
We report the detailed results of using class names from 11 different datasets as anchors in Tab.~R7~(supplementary PDF). 

\review{\nr~\nrr~\nrrrr}{Anchor's number and anchor's pattern.}

We consider that the primary factors affecting performance are the pattern of anchors (as discussed in Figure. 4) and the quantity of anchors. 
Meanwhile, for the Caltech101 dataset, opting for DTD (consisting of 47 categories) as anchors leads to a more substantial enhancement in performance than utilizing ImageNet (consisting 1k categories).
The observation of which anchors' pattern can enhance the performance can be summarized as follows:

$\bullet$ When the marginal distribution of target classes (obtained by averaging all rows of the anchor-target relation matrix) is more balanced, there is a greater potential for performance improvement. 

$\bullet$ It is expected that the probability distribution of anchors across target classes is neither unimodal (such as one-hot encoding) nor uniformly distributed. Having the anchor's similarity distribution across target classes diverse indicates meaningful associations between the anchor and various target classes.

Regarding the learnable scenarios, we posit that a greater quantity of anchors is undoubtedly advantageous, provided that these anchors exhibit favorable patterns learned from the data. Nonetheless, we hypothesize that when dealing with a scarcity of samples, the model's capacity to acquire a significant number of such advantageous anchors could be limited.
% When the number of anchors is substantial, attempting to learn the powerful pattern using only a small number of samples might prove challenging.
% As illustrated in Figure 4(a), for the Caltech101 dataset, opting for DTD (consisting of 47 categories) as anchors leads to a more substantial enhancement in performance than utilizing ImageNet (consisting 1k categories). This observation implies that the powerful pattern of anchors appears to bear heightened importance.

\subsection{Components and parameters}

\review{\nr~\nrrrr}{Implementation of RTM.}
RTM is a standardized transformer layer consisting of a self-attention layer and FNN, which takes the visual feature as ``Query", the text features of the anchors as ``Key" and the similarity matrix between the text features of anchor and target classes as ``Value".
A crucial point to clarify is that we do not concatenate the query, key, and value components together as input to the network. We will provide a comprehensive explanation of this structure in the supplementary material.

\review{\nr~\nrr~\nrrrr}{Parameter and FLOPs comparison.}
MaPle (cvpr23) involves training approximately 3.55M parameters, while RTOS requires around 3.94M parameters, making them roughly comparable in terms of parameter count.
This indicates that having 3-4 million parameters would not pose a burden for CLIP-based few-shot learning.
Furthermore, the parameter count of 3.94M presented in the table includes both the parameters associated with anchors (0.02M) and the parameters for RTM (3.92M).

\review{\nr~\nrrr}{Implementation of image-image relation method.}
The inspiration for the image-image relation method stems from Tip-Adapter-F method.
Tip-Adapter-F utilizes a cache model that stores the features of training images along with their labels in a key-value database. During inference, the feature extracted from a test example is treated as a query, and information is aggregated from the database through retrieval.
Adopting a relation transition perspective, we interpret the cache model's functionality. 
Our aim is to classify a test image by establishing relationships between it and the training images. 
To achieve this, we utilize the training image features as keys and employ the one-hot encoded labels of the training images as the corresponding values of RTM. 
This approach enables us to effectively implement image-image relation transition, ultimately leading to improved classification accuracy.
We apologize for not providing a detailed description of this aspect. We will include a comprehensive explanation of this section in the supplementary materials.

\review{\nr}{Combination of three methods.}
As the combination outcome, we utilize prediction scores derived from three parallel relation transformations:
\begin{equation}
    \mathcal{P}_{final} = \mathcal{P}_{clip} + \alpha^{C} \mathcal{P}_{tar}^{C} + \alpha^{P} \mathcal{P}_{tar}^{P} + \alpha^{I} \mathcal{P}_{tar}^{I}
\end{equation}
where $\mathcal{P}_{tar}^{C}$ is the scores based on the consistency prior, $\mathcal{P}_{tar}^{P}$ is the scores based on the total probability formula, and $\mathcal{P}_{tar}^{I}$ is the scores based on image-image relation.

\subsection{Ablation}

\review{\nrrr}{Zero-shot experiment about different anchors.}
We report the detailed results of using class names from 11 different datasets as anchors in the submitted PDF. 
Additionally, we will include these results in the supplementary materials.
This partial results in Tab.~\ref{tab:r3_major3_details} suggest that Caltech101 is not the best anchor dataset when considering DTD.
The reason for this could be that, as indicated in the second observation of which anchors' pattern can enhance the performance, meeting the requirements of a uniform distribution for $p_{\text{mar.}}^{anc\rightarrow tar} = \{\sum_{j=1}^{C_{anc}} \mathcal{R}_{i,j} \}_{i=1}^{C_{tar}}$ does not necessarily imply achieving a uniform distribution as specified in $p_{\text{mar.}}^{tar\rightarrow anc} = \{\sum_{i=1}^{C_{tar}} \mathcal{R}_{i,j} \}_{j=1}^{C_{anc}}$, where $\mathcal{R}_{i,j} = \dfrac{\exp(\cos( \mathcal{F}_{tar, i},\mathcal{F}_{anc, j} )/\tau)}{
\sum\nolimits_{i=1}^{C_{tar}} \exp(\cos( \mathcal{F}_{tar, i},\mathcal{F}_{anc, j} )/\tau) 
} .$

\review{\nrrr~\nrrrr}{MaPLe and POLT as baseline.}
MaPLe and POLT hold significant positions as baselines, and we deeply regret the oversight of these two methods.
We report the performance and accuracy comparison in Tab.~R1 and Tab.~R2~(supplementary PDF). 

\subsection{Typo and symbol error.}
We will thoroughly review and rectify any such mistakes present in the article.

==> rebuttal/1-HQ1F.tex <==
\review{Major. 1a}{About open-world semantics.}

1) The learnable ``cls" token (anchor) is positioned after the manually designed context prompt ``a photo of", forming ``a photo of \{cls\}". To make the text ``a photo of \{cls\}" meaningful, there exists a high probability that the ``cls" token will represent a semantic. 

2) We say the ``cls" token may represent ``open-world" semantic as the ``cls" token itself is learnable. Theoretically, it can learn to represent arbitrary semantic in the open world. 

3) To demonstrate the possible semantics carried by the anchors, similar to CoOp, we attempt to find the words in WordNet closest to the learned anchors in the embedding space. 
We find that the anchors do carry semantic information in this sense. 
For instance, the closest words include ``lassa", ``choler", ``corday", \emph{etc.} 
As mentioned in CoOp, we cannot make definite conclusions based solely on these observations. Interpreting the learned anchors (``cls" tokens) using the nearest words may not be that accurate, as the semantics represented by the anchors may not perfectly align with the closest words in WordNet.

%Given that anchors undergo random initialization and are subject to training, they are expected to exhibit characteristics aligned with the open-world concept. Additionally, drawing from the "a photo of \{cls\}" learning mechanism, it is reasonable to assume that the acquired anchors are semantic nouns.
%As pointed out in CoOp, interpreting learned anchors presents a formidable challenge, as these vectors might encompass meanings that extend beyond the scope of the existing vocabulary.
%Using a method similar to CoOp, we find in WordNet that the words closest to the learned anchors do indeed carry semantic information. For instance, words like ``lassa", ``choler", and ``corday" are among them.
%, as mentioned in CoOp, we couldn't make definite conclusions based solely on these observations. Interpreting the learned prompts using the nearest words might lead to inaccuracies, as the semantic characteristics of the vectors may not always align perfectly with the closest words.

\review{Major. 1b}{Difference with prompt learning.}
%We apologize for not explicitly clarifying the differences between our method and prompt learning in the paper. We will address this by adding a dedicated section to provide a comprehensive explanation of the distinctions between the two approaches.
1) Comparing the formats of input texts between prompt tuning (``\{learnable token\} [class name]") and ours (``a photo of \{learnable token\}"), it can be seen that the key difference is that we aim to learn the semantic embeddings while the prompt tuning methods aim to learn the context embeddings (\emph{i.e.,} the description content before the semantic nouns).

2) Our relation transition structure is designed for our semantic learning mechanism
and cannot be simply combined with the conventional prompt tuning mechanism,
which also shows the uniqueness of our method compared to prompt tuning. 

%While CoOp operates under the assumption that the learned information is contextual, our approach posits that our learning revolves around category-related insights. Moreover, a distinct emphasis of our method lies in the utilization of relation transitions. We present two theoretically sound techniques for achieving such transitions: one built on the foundation of the consistency prior, and the other grounded in the principles of the total probability formula. The integration of cross-attention mechanisms serves as an expansion of both these transition methods.
3) To further show the uniqueness of our method, we conduct additional experiments. 
We compare our method with the ones which make all the tokens of text input learnable. 
% We compare to two possible solutions, including ``Unified" where all the tokens are independently learned,
% and ``Class-specific" where all the tokens are learnable but partial tokens are shared among different text inputs.
We compare to two possible solutions, including ``Class-specific" where all the tokens are independently learned,
and ``Unified" where all the tokens are learnable but partial tokens are shared among different text inputs.
Results shown below verify the rationality and necessity of our design, showing that our method is different to the conventional prompt tuning method. 
%also carry out a performance evaluation by employing three distinct configurations for the context prompt: unified learnable, class-specific learnable, and "a photo of \{cls\}" frozen.
%\blue{The purpose of this table is to illustrate that our approach and prompt learning methods exhibit differences in terms of performance.}

4) We will add more discussions about the difference between prompt learning and our method in our revised paper.

\begin{table}[h]
    \centering
\scalebox{0.83}{
\begin{tabular}{llllll}
\toprule
Context Prompt     & 1 & 2 & 4 & 8 & 16 \\
\midrule
Unified~(learnable)           & 64.3 & 66.2 & 69.3 & 71.6 & 74.7 \\
Class-specific~(learnable)    & 64.1 & 66.1 & 69.0 & 71.1 & 74.7 \\
``A photo of \{cls\}"~(RTOS-C) & 65.0 & 67.0 & 70.0 & 72.4 & 75.4 \\
\bottomrule
\end{tabular}
}
\vspace{-3mm}
\caption{Average accuracy of 11 datasets. }
\vspace{-3mm}
\label{tab:r1_major_1b}
\end{table}

\review{Major. 1c}{The number of anchors vs. the accuracy.}
Utilizing open semantics doesn't mean the accuracy will consistently increase with the increase of the anchor numbers. The main reason is with the increase of number of anchors, the redundancy of the semantic information provided by different anchors may also increase, which means a infinite number of anchors may not benefit the accuracy improvement. 
We actually verify this in our principle experiment (see Fig. 4). 
E.g., for the Caltech101 dataset, we manually select 47 categories in DTD as anchors, yielding even better results than utilizing 1k categories in ImageNet.



%We consider that the primary factors affecting performance are the quality~(pattern) of anchors (as discussed in Figure. 4) and the quantity of anchors. 
%Meanwhile, for the Caltech101 dataset, opting for DTD (consisting of 47 categories) as anchors leads to a more substantial enhancement in performance than utilizing ImageNet (consisting of 1k categories).
%% The observation in Figure.4 can be concluded as: 
%The observation of which anchors' pattern can enhance the performance can be summarized as follows:
%
%$\bullet$ When the marginal distribution of target classes (obtained by averaging all rows of the anchor-target relation matrix) is more balanced, there is a greater potential for performance improvement. 
%This implies that for the anchor-target relation matrix $\mathcal{R} \in \mathbb{R}^{ C_{tar} \times C_{anc} }$, we expect the marginal distribution $p_{\text{mar.}} = \{\sum_{j=1}^{C_{anc}} \mathcal{R}_{i,j} \}_{i=1}^{C_{tar}}$ to approach a uniform distribution.
%
%$\bullet$ It is expected that the probability distribution of anchors across target classes is neither unimodal (such as one-hot encoding) nor uniformly distributed. Having the anchor's similarity distribution across target classes diverse indicates meaningful associations between the anchor and various target classes.
%This implies that for the anchor-target relation matrix $\mathcal{R} $, we expect any $\mathcal{R}_{:,j}$ is neither unimodal nor uniformly distributed.
%
%\begin{equation}
%     \mathcal{R}_{i,j} = \frac{\exp(\cos( \mathcal{F}_{tar, i},\mathcal{F}_{anc, j} )/\tau)}{
%\sum\nolimits_{i=1}^{C_{tar}} \exp(\cos( \mathcal{F}_{tar, i},\mathcal{F}_{anc, j} )/\tau) 
%} 
%\label{r3_major2_raltion}
%\end{equation}
%
%% As illustrated in Figure 4(a), for the Caltech101 dataset, opting for DTD (consisting of 47 categories) as anchors leads to a more substantial enhancement in performance than utilizing ImageNet (consisting of 1k categories). This observation implies that the powerful pattern of anchors appears to bear heightened importance. When the number of anchors is substantial, attempting to learn the powerful pattern using only a small number of samples might prove challenging.
%
%Regarding the learnable scenarios, we posit that a greater quantity of anchors is undoubtedly advantageous, provided that these anchors exhibit favorable patterns learned from the data. Nonetheless, we hypothesize that when dealing with a scarcity of samples, the model's capacity to acquire a significant number of such advantageous anchors could be limited.

\review{Major. 2}{Concern about zero-shot experiments.}

%\noindent \textbf{Purpose of the report zero-shot experiment.}
%We apologize for any lack of organization in our article's structure. 
%The primary objective of our zero-shot experiments is to conclusively pinpoint the anchor pattern that can benefit the relation transition and final predictions. 
%Our focus is not on achieving state-of-the-art performance for the zero-shot setting.
%The objective is to offer intuitive and theoretical insights into few-shot image classification.
%Given the intrinsic unpredictability and near-impossibility associated with manually selecting anchors for practical applications, we opt to learn anchors under a few-shot setting. In Figure 4(c), we showcase that the learned anchors indeed possess the beneficial patterns we previously observed in the zero-shot setting.

%%\noindent \textbf{Anchors' selection on zero-shot setting.}
1) Our method is not tailored for the zero-shot setting (as the title indicates). 
And we aim not to show the superiority of our method under zero-shot setting. 
We demonstrate the zero-shot results just to show the benefits of the anchor-target relation modeling and the limitations of manually selecting the anchors. 

2) We observe that using anchors generally benefit the zero-shot performance. 
Compared to the improvement brought by manually selecting anchors, 
the improvement brought by random initialization is limited. 
This just verifies that the selection of anchors does matter considering the classification performance. 
This actually motivates us to learn the optimal semantics openly rather than manually select them in the few-shot setting. 

3) We introduce how to select the anchors in the caption of Tab. 1. 
%We apologize for not providing a detailed explanation of the anchor pool. 
For instance, we have 11 datasets. Concerning the Caltech101 dataset, we perform zero-shot testing using class names from the other ten datasets as anchors. 
We then select anchors with the highest performance from those ten datasets, which are presented as the ``selected" results in Tab. 1.
We will add those details in our revised paper.

\review{Minor. 1}{Typo error in Eq. 5.}
$\mathcal{P}$ should be modified to $\mathcal{P}_{tar}$. We will correct it in our revision.
% We sincerely apologize for any typo errors. We will thoroughly review and rectify any such mistakes present in the article.
% The correct expression is
% \begin{equation*}
%     \mathcal{P}_{tar} = \frac{
%     \exp( \cos(\mathcal{P}_{anc}, \mathcal{R}) / \tau' )
%     }{
%     \sum_{i=1}^{C_{tar}} \exp( \cos(\mathcal{P}_{anc}, \mathcal{R}_{i}) / \tau' )
%     } ,
% \end{equation*}
% where image-target relation $\mathcal{P}_{tar} \in \mathbb{R}^{C_{tar}}$.

\review{Minor. 2}{Details of the transformer architecture.}
RTM is a standard transformer layer consisting of a self-attention layer and FNN, which takes the visual feature as ``Query", the text features of the anchors as ``Key" and the similarity matrix between the text features of anchor and target classes as ``Value".
We provide relevant data in the table below for your reference.

\begin{table}[h]
\begin{center}
\scalebox{1}{
\begin{tabular}{lcccc}
\hline
Method(ViT16)&Shots & Tuned Params  & Acc  \\ \hline
MaPLe(cvpr23)&1     & 3.55M         & 69.7 \\
Tip-Adapter-F&1     & 0.82M         & 71.3 \\
Ours         &1     & 3.94M         & 71.8 \\ \hline
MaPLe        &16    & 3.55M         & 81.2 \\
Tip-Adapter-F&16    & 8.19M         & 81.1 \\
Ours         &16    & 3.94M         & 81.3 \\ \hline
\end{tabular}
}
\end{center}
\vspace{-3mm}
\caption{Comparison of computational complexity among different methods~(ViT-B/16). Acc denotes the average accuracy of 11 datasets.}
\vspace{-3mm}
\end{table}

\review{Minor. 3}{Combination of three methods.}

% The inspiration for the image-image relation method stems from Tip-Adapter-F method.
% Tip-Adapter-F utilizes a cache model that stores the features of training images along with their labels in a key-value database. During inference, the test image feature is treated as a query, and information is aggregated from the database through retrieval.
% We interpret the cache model by adopting a relation transition perspective. 
% Our aim is to classify a test image by establishing relationships between it and the training images. 
% To achieve this, we utilize the training image features as keys and employ the one-hot encoded labels of the training images as the corresponding values of RTM. 
% This approach enables us to implement image-image relation transition, ultimately improving classification accuracy.
% We apologize for not providing a detailed description of this aspect. We will include a comprehensive explanation of this section in the supplementary materials.

Sorry for this confusion. 
We combine three methods by averaging the prediction scores obtained from them.
Tab. 3 should be cited at the end of the method section when discussing the three types of realizations.
We will clarify this in our revised version.
%As the combination outcome, we utilize prediction scores derived from three parallel relation transformations:
%\begin{equation}
%    \mathcal{P}_{final} = \mathcal{P}_{clip} + \alpha^{C} \mathcal{P}_{tar}^{C} + \alpha^{P} \mathcal{P}_{tar}^{P} + \alpha^{I} \mathcal{P}_{tar}^{I}
%\end{equation}
%where $\mathcal{P}_{tar}^{C}$ is the scores based on the consistency prior, $\mathcal{P}_{tar}^{P}$ is the scores based on the total probability formula, and $\mathcal{P}_{tar}^{I}$ is the scores based on image-image relation.

%In accordance with the reviewer's suggestion, Tab.3 will be cited at the end of the method section when discussing the three types of relation-transmission methods.

==> rebuttal/2-5zSa.tex <==
\review{Major. 1}{Concern about the novelty.}
There exist some misunderstandings. 
We don't introduce additional model to tune the large model. 
We admit that we introduce additional training parameters, but most previous works tailored for this setting including CoOp, MaPLe and Tip-Adapter do introduce additional training parameters (see the comparison shown in table below).
In CoOp, the context prompt is learned, while in ours, the open semantics are learned.
Our RTM module is designed to help learn and utilize the open semantics from CLIP.
In this sense, we believe the performance gain largely comes from the fact that we extract more useful knowledge from CLIP via our learning mechanism to facilitate the few-shot learning. 


%Our method approaches image classification from the standpoint of relation transitions, with the goal of enhancing prediction performance through open semantic relation transitions. 
%The data displayed in the table below serves to demonstrate that the additional parameter count introduced by our model is well within a reasonable and acceptable range.
%Unlike parameter tuning, our primary objective is to leverage the inherent semantic relations present in the CLIP model to enrich predictions in a few-shot setting.
% We are sincerely grateful for the thoughtful insights you've shared. 
% While we recognize the viewpoint that our approach involves an additional model for fine-tuning, it's important to emphasize that our method differs from parameter tuning.
% Our approach is designed to leverage open semantics through relation transitions.
% The data displayed in the table below serves to demonstrate that the additional parameter count introduced by our model is well within a reasonable and acceptable range.

% Our method centers around the concept of relation transitions, which aims to enhance prediction performance through open semantic relation transitions. 
% Unlike parameter tuning, our primary objective is to leverage the inherent semantic relations and patterns present in the CLIP model to enrich predictions in a few-shot setting.

% It's pertinent to highlight that our focus is on identifying anchor patterns within relation transitions, and these patterns play a pivotal role in guiding the model's predictions. We do not merely rely on parameter adjustments; instead, we empower the model to learn how to transition between semantic relations and make informed predictions.

% We understand your concern about the performance gains and the influence of dataset-specific biases versus CLIP's inherent knowledge. Our approach aims to strike a balance by utilizing both the knowledge of the CLIP model and the learned patterns specific to the task at hand.

% We hope this explanation provides a clearer perspective on our method.

% In our perspective, the fundamental principle of transfer learning involves preserving the knowledge acquired from the source domain while harnessing the insights gained from the target domain. 
% \red{TODO: ...}

\begin{table}[h]
\begin{center}
\scalebox{1}{
\begin{tabular}{lcccc}
\hline
Method(ViT16)&Shots & Tuned Params  & Acc  \\ \hline
MaPLe(cvpr23)&1     & 3.55M         & 69.7 \\
Tip-Adapter-F&1     & 0.82M         & 71.3 \\
Ours         &1     & 3.94M         & 71.8 \\ \hline
MaPLe        &16    & 3.55M         & 81.2 \\
Tip-Adapter-F&16    & 8.19M         & 81.1 \\
Ours         &16    & 3.94M         & 81.3 \\ \hline
\end{tabular}
}
\end{center}
\vspace{-3mm}
\caption{Comparison of the amount of tuned parameters and accuracy among different methods~(ViT-B/16). Acc denote the average accuracy of 11 datasets.}
\vspace{-3mm}
\label{tab:r2_major1_cpr_params_}
\end{table}

\review{Major. 2}{Difference with methods based on autocorrelation matrix.}
%We apologize for not clarifying the distinctions between our approach and previous methods based on autocorrelation matrix.
As the reviewer didn't suggest any specific papers to compare with, we survey more papers, trying to find papers sharing similar ideas. But as far as we know, there are no previous works trying to mine the open semantics and perform the few-shot learning via the relation transition between the open semantics and the target classes.
We think the reason is that without CLIP and carefully designed mechanism, it is impossible to effectively mine the open semantics and utilize them to perform the few-shot learning. 
Thus, we believe that we make novel and enough contributions.

% TODO: the following description is too complex for the reviewer to understand. 
%In previous covariance-based few-shot learning methods, such as CovaMNet~[a], the features are obtained from the support set. These support image features, which play a pivotal role in classification, align with the features of target categories. If measured using CLIP, the similarity distribution between any support set's image features and the target categories should exhibit an unimodal distribution. Methods of this nature rely on features that align with the target categories.
%
%As discussed in the "Effect of different choices of anchors" subsection, we anticipate that anchors beneficial for enhancing model performance should not adhere to an unimodal similarity distribution with target categories. Instead, we seek to learn diverse anchors, and the associated similarity distribution should not be uniformly distributed.
%
%From our perspective, the zero-shot branch of CLIP appears to be more conceptually aligned with previous methods, as the features learned from text categories in CLIP can be viewed as an expectation of the support set image features in prior methods. In contrast, our approach aims to enhance CLIP's classification performance by learning features distinct from target categories through relation transition. Furthermore, based on our understanding, the relation transition in covariance-based methods seems to differ from our approach's relation transition. This discrepancy might be attributed to our limited knowledge, and we welcome the reviewer to point out similar methodologies if they exist.
%
%Additionally, our method is rooted in CLIP. Our objective revolves around exploring the open semantics constructed by CLIP to enhance model predictions. Thus, from a macro perspective, our starting point diverges from previous approaches that rely on support image sets.
%
%We hope this explanation addresses any concerns you may have, esteemed reviewer.

%\noindent[a] Distribution consistency based covariance metric networks for few-shot learning

\review{Major. 3}{More broader tasks.}
As suggested, we verify our method on the few-shot semantic segmentation task. 
%We posit that the approach based on RTOS could also be applicable to semantic segmentation.
We evaluated the segmentation performance on the VOC2012 dataset using a subset of 65 images. This subset was carefully selected to ensure that each class is represented in approximately 4 images. These images were used to form the training set, while the VOC2012 validation set was employed for validation purposes. We employed an RN50 backbone. 
%with a configuration that involved resizing the shorter side of the images to 320 pixels, aiming for rapid verification of the method's effectiveness. 
To achieve semantic segmentation results, we modified the Global Attention Pooling of the final layer in the RN50 CLIP model following the paradigm of MaskCLIP.
This experiment demonstrates that our approach outperforms the CLIP baseline (``ZSCLIP") and the typical prompt tuning method CoOp remarkably.

\begin{table}[h]
\begin{center}
\begin{tabular}{llll}
\hline
     & ZS-CLIP & CoOp & Ours \\ \hline
mIoU & 18.6           & 19.6 & 21.5   \\ \hline
\end{tabular}
\end{center}
\vspace{-3mm}
\caption{Semantic Segmentation Performance on VOC2012 with mIoU Metric.}
\vspace{-3mm}
\end{table}

\review{Major. 4}{Parameter and FLOPs comparison.}
%We apologize for the omission of the parameter and FLOPs comparison. 
%MaPle (cvpr23) involves training approximately 3.55M parameters, while RTOS requires around 3.94M parameters, making them roughly comparable in terms of parameter count.
%This indicates that having 3-4 million parameters would not pose a burden for CLIP-based few-shot learning.
%Returning to the reviewer's question, the parameter count of 3.94 million presented in the table encompasses both the parameters related to anchors (0.02 million) and those for RTM (3.92 million).
%We will report Tab.~\ref{tab:r2_major1_cpr_params_} and Tab.~\ref{tab:r2_major4_cpr_params_} in the supplementary materials.
As suggested, we present the parameters and the FLOPS comparisons below. It can be seen that the induced memory and speed complexity is comparable to previous state-of-the-arts in general.


\begin{table*}
\begin{center}
\begin{tabular}{lllllll}
\hline
Methods          & Backbone & Training Cost & GFLOPs & Params  & Infer. Speed & GPU Memory \\ \hline
Zero-shot CLIP   & RN50     & 0             & 6.14   & 39.34M  & 11.85ms      & 1648MiB    \\
CoOp             & RN50     & 880min        & 6.14   & 39.34M  & 11.85ms      & 1648MiB    \\
Synthetic        & RN50     & -             & 6.14   & 39.34M  & 11.85ms      & 1648MiB    \\
CLIP-Adapter     & RN50     & 50min         & 6.14   & 39.87M  & 12.00ms      & 1650MiB    \\
Tip-Adapter-F    & RN50     & 5min          & 6.17   & 71.72M  & 12.06ms      & 1776MiB    \\
PLOT             & RN50     & -             & 9.31   & 92.22M  & 29.59ms      & 2908MiB    \\
Ours             & RN50     & 5min          & 6.32   & 53.10M  & 12.77ms      & 1702MiB    \\ \hline
Zero-shot CLIP   & ViT-B16  & 0             & 17.58  & 86.70M  & 10.40ms      & 1710MiB    \\
CoOp             & ViT-B16  & 1724min       & 17.58  & 86.70M  & 10.40ms      & 1710MiB    \\
Synthetic        & ViT-B16  & -             & 17.58  & 86.70M  & 10.40ms      & 1710MiB    \\
CLIP-Adapter     & ViT-B16  & 73min         & 17.58  & 86.84M  & 10.66ms      & 1710MiB    \\
Tip-Adapter-F    & ViT-B16  & 7min          & 17.61  & 110.90M & 10.69ms      & 1804MiB    \\
MaPLe            & ViT-B16  & 66min         & 17.77  & 86.72M  & 11.08ms      & 1710MiB    \\
Ours             & ViT-B16  & 8min          & 17.65  & 90.74M  & 11.23ms      & 1716MiB    \\ \hline
\end{tabular}
\end{center}
\vspace{-3mm}
    \caption{
    Comparison of time efficiency for different methods on 16-shot ImageNet.
    All experiments are tested with batch size 1 on a single NVIDIA Tesla V100 GPU.
    \textcolor{red}{Among these metrics, excluding the Training Cost, none account for the text encoder's forward propagation process. 
    For example, during the inference stage of CoOp, only the extracted text features are utilized as classification weights.}
    }
\label{tab:r2_major4_cpr_params_}
\vspace{-3mm}
\end{table*}

==> rebuttal/2r1-5zSa.tex <==
We would like to express our gratitude for the substantial time and valuable feedback provided by the reviewer. 
We respect the decision.
But, we request the opportunity to provide our different opinions and additional insights.


\textbf{Q1: Difference with previous prompt tuning methods.}

Thanks for the reviewer's comments. 

1) Freezing CLIP and tuning additional parameters to adapt to few-shot tasks is just a very general paradigm. We follow this paradigm, but this doesn't mean we make no valuable contributions. 

2) As we emphasized in our previous rebuttal, previous works choose to tune the \textit{prompt} (\emph{i.e.,} the context) of text input, while we don't tune the prompt but make the semantics learnable. 
This seemingly simple modification yields substantially different learning mechanisms. 
From the technical view, in prompt tuning, as the class token of text input is fixed and aligned with target class, we may directly compare the image features to the text features of different classes to make predictions.
But this way cannot be trivially transferred to our framework as 
the class token of the text input is learnable and not necessarily aligned with the target class. 
This technical difference actually reflects different ways to utilize the knowledge encoded in the CLIP. 
That is, prompt-tuning methods aim to tune the \textit{context} of text input to make the class-specific textural features more aligned with image features,
while ours aim to mine relationships between target class and open semantics to facilitate few-shot learning.
We believe our new perspective is at least a valuable supplement to existing prompt-tuning methods. 


\textbf{Q2: The novelty.}

Thanks for the reviewer's detailed comments. Our opinions regarding differences with the suggested papers are as follows 

1) From a high-level, our method shares some similarities with previous works [1-3] which utilize the class-wise relationships in classification. But the key difference between previous works and ours is that 
previous works only consider relationships within a close target class set,
while the anchor class in our method is ``open".

2) The design of mining ``open" semantics is enabled by CLIP. 
%That is why we claim that we extract useful knowledge from CLIP.
On one hand, our paper answers how to utilize the relationships between target classes and \textit{open semantics} with the aid of CLIP;
on the other hand, we provide a new perspective regarding what kind of knowledge can be mined from CLIP to benefit the downstream few-shot learning tasks.
%Our unique contribution is that we answer how to utilize the relationships between target classes and \textit{open semantics} with the aid of CLIP.
Those two aspects are our unique contributions and make our method distinct with previous works [1-3] and previous prompt-tuning methods.

%2) From another perspective, CLIP encoders abundant multi-modal knowledge. Extracting or utilizing what kind of knowledge from CLIP remains an open question. Previous prompt-tuning method is one possible way. 
%^We provide another way. 


\textbf{Q3: Insufficient experiments.}

Thanks for your suggestions. 

1) Identical to previous related works \textcolor{red}{[8,10,11,29,32]} cited in our paper, we make comparisons on 11 benchmarks. The superior results sufficiently justify the effectiveness of our method in the typical few-shot setting where training images and test images are within the same domain.  

2) We also noticed that several works like \textcolor{red}{[8, 9, R1]} also report the few-shot learning results under domain/distribution shift. During rebuttal, we make additional experiments. The results below show our method outperforms previous prompt-tuning methods remarkably. 

3) As shown in previous rebuttal, we also compare our method to previous prompt-tuning methods on the few-shot semantic segmentation task. The results also justify the effectiveness of our method.

[R1] MaPLe: Multi-modal Prompt Learning (cvpr23)

%\textbf{1. Comparison with prompt tuning methods.}
%In contrast to prompt tuning methods, our approach primarily focuses on performance within the target domain.
%We regret that our method and its performance fall short of leaving a favorable impression on the reviewer.
%% 感觉这个审稿人没办搞定，就随便答了，让他不回了就行了？
%
%\textbf{2. Concerning the novelty.}
%Indeed, our approach shares conceptual similarities with the methods mentioned by the reviewer. Furthermore, we seek clarification on your remarks regarding soft labels.
%
%a. 
%Assuming that you consider the transformation of relations as a form of soft label conversion. It is true that manually designed soft labels unavoidably introduce additional noise. 
%However, unlike the soft labels obtained through label smoothing and the heuristic soft labels discussed in [2], the relations derived from our method via transition are inherently learnable. 
%Should the noise introduced by manually designed soft labels be attributed to the non-learnable nature of this approach?
%
%b. 
%If your concern relates to our utilization of label smoothing loss in our code implementation rather than cross-entropy loss, we acknowledge that we did indeed employ label smoothing loss here, resulting in a moderate performance enhancement. 
%Nonetheless, this improvement is not substantial. 
%If necessary, we are prepared to provide supplementary ablation studies for this aspect.
%
%\textbf{3. About more experiments.}
%As mentioned above, in contrast to prompt tuning methods, our approach primarily focuses on performance within the target domain.
%As a result, we have not conducted certain experiments concerning model generalization. 
%However, as mentioned by the reviewer, we did indeed overlook certain experiments. 
%In the table below, we report the robustness experiments of our method.

\begin{table}[]
\begin{tabular}{llllll}
\hline
\multirow{2}{*}{Method} & Source        & \multicolumn{4}{c}{Target}                                    \\ \cmidrule(lr){2-3} \cmidrule(lr){3-6}
                        & ImageNet      & -V2           & -S            & -A            & -R            \\ \hline
CLIP                    & 66.7          & 60.8          & 46.2          & 47.8          & 74.0          \\
CoOp                    & 71.5          & 64.2          & 48.0          & 49.7          & 75.2          \\
CoCoOp                  & 71.0          & 64.1          & 48.8          & 50.6          & 76.2          \\
MaPLe                   & 70.7          & 64.1          & \textbf{49.2} & 50.9          & 77.0          \\
Ours                    & \textbf{73.5} & \textbf{66.1} & \textbf{49.2} & \textbf{51.0} & \textbf{78.0} \\ \hline
\end{tabular}
\caption{
The robustness (\%) to distribution shift of different methods~(ViT-B/16). 
}
\end{table}
% 有些论文有base2new的实验，但是这个我们的方法实现不了。

%All in all, we would like to extend our gratitude once again for the valuable insights provided by the reviewer. 
%We also understand and respect the decision not to modify the score. 
%Thanks.

Finally, we respect the reviewer's effort in providing detailed comments. We sincerely hope the reviewer can examine our opinions and reconsider the rating. If the reviewer has any further questions or concerns, we are willing to answer them.

==> rebuttal/3-JQvo.tex <==
\review{Major. 1}{The motivation and implementation of image-image relation method.}
The motivation for the image-image relation method stems from Tip-Adapter.
Tip-Adapter utilizes a cache model that stores the features of training images along with their labels in a key-value database. During inference, the feature extracted from a test example is treated as a query, and information is aggregated from the database through retrieval.
We leverage training image features along with their corresponding labels from a relational transition perspective.
Our aim is to classify the test image by establishing relationships between it and the training images. 
To achieve this, we utilize the training image features as keys and employ the one-hot encoded labels of the training images as the corresponding values of RTM. 
This approach enables us to implement image-image relation transition, ultimately improving classification accuracy.
We will include a comprehensive explanation in our revised paper.


\review{Major. 2}{Anchor pool and guideline to select anchors.}

1) \noindent\textbf{Anchor pool:} 
The anchor pool refers to the set of class names defined in 11 datasets utilized in the paper.
Concerning the Caltech101 dataset, we perform zero-shot testing using class names from the other ten datasets as anchors. 
We then select anchors with the highest performance from those ten datasets, which are presented as the ``selected" results in Tab. 1.
We will add those details in our revised paper.
% We mentioned the anchor pool in the caption of Table 1, ``The class names of anchors are chosen from the class definitions in the other 10 datasets." 
% We apologize for not providing a detailed explanation of the anchor pool. 
% For instance, concerning the Caltech101 dataset, we perform zero-shot performance testing using class names from the other ten datasets as anchors. 
% We then select anchors with the highest performance from those ten datasets, which are presented as the ``selected" results in Table. 1.
% \blue{Your conjecture in Major 3 is accurate.}
% We will supplement the detailed explanation of this aspect in the supplementary materials.

2) \noindent\textbf{Powerful pattern which may benefit the relation transition: }
Within the range of lines 264 to 270, we discussed which anchor pattern may benefit relation transitions and final predictions.
We have observed the following:

- When the marginal distribution of target classes (obtained by averaging all rows of the anchor-target relation matrix) is more balanced, there is a greater potential for performance improvement. 
% This implies that for the anchor-target relation matrix $\mathcal{R} \in \mathbb{R}^{ C_{tar} \times C_{anc} }$, we expect the marginal distribution $p_{\text{mar.}} = \{\sum_{j=1}^{C_{anc}} \mathcal{R}_{i,j} \}_{i=1}^{C_{tar}}$ to approach a uniform distribution.

- It is expected that the probability distribution of anchors across target classes is neither unimodal (such as one-hot encoding) nor uniformly distributed. 
% Having the anchor's similarity distribution across target classes diverse indicates meaningful associations between the anchor and various target classes.
% This implies that for the anchor-target relation matrix $\mathcal{R} $, we expect any $\mathcal{R}_{:,j}$ is neither unimodal nor uniformly distributed.

% \begin{equation}
%      \mathcal{R}_{i,j} = \frac{\exp(\cos( \mathcal{F}_{tar, i},\mathcal{F}_{anc, j} )/\tau)}{
% \sum\nolimits_{i=1}^{C_{tar}} \exp(\cos( \mathcal{F}_{tar, i},\mathcal{F}_{anc, j} )/\tau) 
% } 
% \label{r3_major2_raltion}
% \end{equation}

3) \noindent\textbf{Our way to select anchors:} 
% For manual selection of anchors, it is possible that we introduce noise rather than useful knowledge.
% As discussed in Line 264-270, the arbitrary selection of anchors doesn't necessarily improve the classification accuracy. 
% However, we find that the anchors that benefit the classification do exist. 
% Thus, the problem lies in how to select the effective anchors. 
% As carefully manual selection is costly and not general, we choose to learn the anchors.
As careful manual selection is costly and not general, we choose to learn the anchors.
As illustrated in Fig 4.(c), the learned anchors exhibit the desired pattern that we expect anchors to possess.

\review{Major. 3}{More ablations about different anchors}
%1) \noindent\textbf{Details of anchor pool}: 
%Indeed, we chose the class names from the remaining ten datasets from eleven datasets, excluding the dataset used for testing, to serve as anchors. 
%We then select anchors with the highest performance from those ten datasets, which are presented as the ``selected" results in Tab. 1.
%We will provide a detailed explanation in our revised paper.
% Among these, we selected the group of anchors that demonstrated the highest performance and reported it in Table 1. 
%2) \noindent\textbf{Ablation about different anchors}:
We report the detailed results of using class names from 11 different datasets as anchors in Tab. R7~(supplementary PDF). 
The partial results in Tab.~\ref{tab:r3_major3_details} suggest that Caltech101 is not the best anchor dataset when considering DTD.
The reason for this could possibly be that the two conditions discussed in Major. 2 are not equivalent when transitioning from anchor to target and from target to anchor.
We will include these results in the supplementary materials.
% The reason for this could be that, as indicated in the second observation of [Major.2], meeting the requirements of a uniform distribution for $p_{\text{mar.}}^{anc\rightarrow tar} = \{\sum_{j=1}^{C_{anc}} \mathcal{R}_{i,j} \}_{i=1}^{C_{tar}}$ does not necessarily imply achieving a uniform distribution as specified in $p_{\text{mar.}}^{tar\rightarrow anc} = \{\sum_{i=1}^{C_{tar}} \mathcal{R}_{i,j} \}_{j=1}^{C_{anc}}$.
% The same holds true for the second observation.

\begin{table}[h]
\begin{center}
\begin{tabular}{lccccc}
\hline
\rotatebox{70}{Anchors} & \rotatebox{70}{FGVCAircraft} & \rotatebox{70}{SUN397} & \rotatebox{70}{OxfordPets} & \rotatebox{70}{ImageNet} & \rotatebox{70}{Caltech101} \\\hline
Accuracy       & 43.3 & 43.2   & 43.2         & 43.1     & 43.0        \\
\hline
\end{tabular}
\end{center}
\caption{Accuracy on DTD dataset with different datasets as anchors.}
\label{tab:r3_major3_details}
\end{table}

\review{Major. 4}{More anchors could lead to worse performance.}
%Utilizing open semantics doesn't mean the accuracy will consistently increase with the increase of the anchor numbers.
The main reason is with the increase of number of anchors, the redundancy of the semantic information provided by different anchors may also increase, which means a infinite number of anchors may not benefit the accuracy improvement. 
We actually verify this in our principle experiment (see Fig. 4). 
E.g., for the Caltech101 dataset, we manually select 47 categories in DTD as anchors, yielding even better results than utilizing 1k categories in ImageNet.
%We consider that the primary factors affecting performance are the quality(pattern) of anchors (as discussed in [Major.2]) and the quantity of anchors. 
%% When the number of anchors is substantial, attempting to learn the powerful pattern using only a small number of samples might prove challenging.
%As illustrated in Figure 4(a), for the Caltech101 dataset, opting for DTD (47 categories) as anchors leads to a more substantial enhancement in performance than utilizing ImageNet (1k categories). 
%
%Regarding the learnable scenarios, we posit that a greater quantity of anchors is undoubtedly advantageous, provided that these anchors exhibit desired favorable patterns learned from the data. 
%We think that when dealing with a scarcity of samples, the model's capacity to acquire a significant number of such desired anchors could be limited.

\review{Major. 5}{Dataset-specific accuracy in Tab. 2}
In Fig. 3, we actually show the required information. 
For clarification, we will list the numbers in tables in the supplementary material.

\review{Major. 6}{MaPLe as baseline}
As suggested, we conduct experiments to compare to MaPLe and show the results below. 
The image encoder of CLIP we used is ViT-B/16.
%We increased the training epochs for the Maple method to 10 and 20 to achieve better performance and replicated the results of several other baselines on the ViT-B/16 backbone, which be reported as follows. 
% We inadvertently omitted to include Maple as one of the baseline methods.

\begin{table}[h]
\centering
\begin{tabular}{lccccc}
\toprule
method           & 1    & 2    & 4    & 8    & 16   \\
\midrule
% CoOp             & 67.6 & 70.3 & 73.6 & 76.4 & 79.3 \\
% CoCoOp           & 68.7 & 70.4 & 71.7 & 73.7 & 75.7 \\
Tip-Adapter      & 71.3 & 73.4 & 76.1 & 78.9 & 81.1 \\
% MaPLe-XD       & 65.1 & 64.8 & 67.5 & 69.3 & 71.5 \\
MaPLe            & 67.5 & 70.8 & 72.7 & 76.3 & 78.4 \\
MaPLe~(10~epoch) & 69.4 & 73.8 & 76.3 & 78.5 & 81.1 \\
MaPLe~(20~epoch) & 69.7 & 73.7 & 76.2 & 78.4 & 81.2 \\ 
% \rowcolor[gray]{.9}
% RTOS             & 71.8 & 73.9 & 76.4 & 78.8 & 81.3 \\
\rowcolor[gray]{.9}
% RTOS-IR        & 72.4 & 74.3 & 76.9 & 79.6 & 82.1 \\
Ours          & \textbf{72.4} & \textbf{74.3} & \textbf{76.9} & \textbf{79.6} & \textbf{82.1} \\
\bottomrule
\end{tabular}
\caption{
\textbf{Average accuracy of 11 datasets.}
The image encoder of CLIP is ViT-B/16.
}
\label{tab:my_label}
\end{table}

\review{Minor. 2}{Title should have broader coverage.}
Sorry for this confusion.
Our method is not tailored for the zero-shot setting (as the title indicates). 
And we aim not to show the superiority of our method under zero-shot setting. 
We demonstrate the zero-shot results just to show the benefits of the anchor-target relation modeling and the limitations of manually selecting the anchors, which motivates our design of learnable anchor-target relation modeling.
%The zero-shot method, which necessitates manual anchor selection, may prove impractical for real-world applications.
%The objective is to offer intuitive insights into image classification within a few-shot setting.
%Our intent in reporting the results of the zero-shot evaluation primarily revolves around two key points:
%
%- To emphasize that, relative to the number of anchors, the desired favorable pattern of anchors may more significantly impact performance.
%
%- As depicted in Fig. 4, we seek to explore which pattern of anchors contributes to performance improvement. Additionally, we aim to validate whether the anchors learned during the few-shot process exhibit the desired favorable anchor pattern.

We will make this clearer in our revised paper. 

\review{Minor. 1\&3\&4}{Typo and symbol errors.}
Thanks. We will correct it in our revision.

% \review{Minor. 4}{Symbol Error.}
% Thank you for your guidance. We will make the necessary corrections to accurately represent the symbols in question.
% \blue{\sout{The description provided here seems appropriate, and I will revisit it later for confirmation.}}

==> rebuttal/4-LDc8.tex <==
\review{Major. 1}{Concern about the motivation.}
For manual selection of anchors, it is possible that we introduce noise rather than useful knowledge.
As discussed in Line 264-270, the arbitrary selection of anchors doesn't necessarily improve the classification accuracy. 
However, we find that the anchors that benefit the classification do exist. 
Thus, the problem lies in how to select the effective anchors. 
As carefully manual selection is costly and not general, we choose to learn the anchors.
%This is why we choose to learn the anchors.
%Lines 264-270 encompass a discussion on the essential characteristics that powerful anchors ought to possess. In alignment with the reviewer's perspective, the arbitrary introduction of anchors does not inherently enhance performance. Hence, we pursued the avenue of learning anchors in a few-shot setting. This process of learning is exemplified in Figure 4(c), wherein we illustrate that the acquired anchors exhibit, to a significant extent, the distinctive patterns that we associate with potent anchors.

%\noindent\textbf{The observation.} 
%We discussed the powerful pattern to enhance relation transitions and final predictions in lines 264-270. We have observed the following:
%
%$\bullet$ When the marginal distribution of target classes (obtained by averaging all rows of the anchor-target relation matrix) is more balanced, there is a greater potential for performance improvement. 
%This implies that for the anchor-target relation matrix $\mathcal{R} \in \mathbb{R}^{ C_{tar} \times C_{anc} }$, we expect the marginal distribution $p_{\text{mar.}} = \{\sum_{j=1}^{C_{anc}} \mathcal{R}_{i,j} \}_{i=1}^{C_{tar}}$ to approach a uniform distribution.
%
%$\bullet$ It is expected that the probability distribution of anchors across target classes is neither unimodal (such as one-hot encoding) nor uniformly distributed. Having the anchor's similarity distribution across target classes diverse indicates meaningful associations between the anchor and various target classes.
%This implies that for the anchor-target relation matrix $\mathcal{R} $, we expect any $\mathcal{R}_{:,j}$ is neither unimodal nor uniformly distributed.
%
%\begin{equation}
%     \mathcal{R}_{i,j} = \frac{\exp(\cos( \mathcal{F}_{tar, i},\mathcal{F}_{anc, j} )/\tau)}{
%\sum\nolimits_{i=1}^{C_{tar}} \exp(\cos( \mathcal{F}_{tar, i},\mathcal{F}_{anc, j} )/\tau) 
%} 
%\label{r3_major2_raltion}
%\end{equation}

\review{Major. 2}{Details about the RTM.}

1) Sorry for making you confused about our RTM.
RTM is a typical transformer encoding layer consisting of a self-attention layer and a FFN, which takes the visual feature as ``Query", the text features of the anchors as ``Key" and the similarity matrix between the text features of anchors and target classes as ``Value".
A crucial point to clarify is that we do not concatenate the query, key, and value components together as input to the network. We will provide a comprehensive explanation of this structure in our revised paper. 
%We apologize for not providing a detailed explanation of this architecture earlier.

2) We make a comparison between our method and previous state-of-the-arts in terms of the amount of learnable parameters and the corresponding accuracy, as shown in the table below.
We observe that we don't introduce too much parameters and achieve better results. 
For example, under the 1-shot setting, the amount of learnable parameters for our method are comparable to that for MaPLe (3.94M vs. 3.55M), but the accuracy of ours is much higher than MaPLe (71.8 vs. 69.7).
We hope those numbers can address the reviewer's concern.

%\noindent\textbf{Parameters of RTM.}
%We understand the concern raised by the reviewer.
%MaPle (cvpr23) involves training approximately 3.55M parameters, while RTOS requires around 3.94M parameters, making them roughly comparable in terms of parameter count.
%Furthermore, it's important to note that the parameter count of 3.94M presented in the table includes both the parameters associated with anchors (0.02M) and the parameters for RTM (3.92M).
%We hope this information adequately addresses the reviewer's concern.

\begin{table}[h]
\begin{center}
\scalebox{1}{
\begin{tabular}{lcccc}
\hline
Method(ViT16)&Shots & Tuned Params  & Acc  \\ \hline
MaPLe(cvpr23)&1     & 3.55M         & 69.7 \\
Tip-Adapter-F&1     & 0.82M         & 71.3 \\
Ours         &1     & 3.94M         & 71.8 \\ \hline
MaPLe        &16    & 3.55M         & 81.2 \\
Tip-Adapter-F&16    & 8.19M         & 81.1 \\
Ours         &16    & 3.94M         & 81.3 \\ \hline
\end{tabular}
}
\end{center}
\vspace{-3mm}
\caption{Comparison of computational complexity among different methods~(ViT-B/16). Acc denote the average accuracy of 11 datasets.}
\vspace{-3mm}
\end{table}

\review{Major. 3}{The work is not complete.}
This is a misunderstanding. In our method, the anchors are learnable rather than manually selected. 
We show the manually selection results under the zero-shot setting in Table 1 just to analyze the effect of anchor selection and illustrate the necessity of making the anchors learnable.
But as the title indicates, we don't focus on the zero-shot setting and aim not to show the superiority of our method under zero-shot setting.
%The zero-shot approach, which necessitates manual anchor selection, may prove impractical for real-world applications. Our intent in reporting the results of the zero-shot evaluation primarily revolves around two key points:
%
%$\bullet$ To emphasize that, relative to the quantity of anchors, the characteristics of anchors also significantly impact performance.
%
%$\bullet$ As depicted in Figure 4, we seek to explore which attributes of anchors contribute to performance improvement. Additionally, we aim to validate whether the anchors learned during the few-shot process exhibit the desirable properties we expect from effective anchors.
%
%We apologize for any lack of clarity in the articulation of our article's structure. We will revise this aspect to better reflect our intentions and highlight the core ideas we wish to convey. 

\review{Major. 4}{Missing of baseline PLOT.}
Thanks for the suggestion. 
We perform the comparison with PLOT below based on ResNet50.
The numbers show that our method is comparable to PLOT.
%We regret the omission of the PLOT baseline and assure you that we will provide the necessary data for this method in Tab.~\ref{tab:r4_major4_comparison_on_fewshot} and Tab.~\ref{tab:r4_major4_polt}.
%We will reproduce and provide the missing results for PLOT with ViT-B/16.
We will add more comparison to PLOT in our revised paper.

\begin{table}[h]
\begin{center}
\scalebox{1.0}{
\begin{tabular}{lccccc}
\toprule[1pt]
\multicolumn{1}{c}{\multirow{2}{*}{Method}} & \multicolumn{5}{c}{Number of shots} \\
\cmidrule(lr){2-6}
                        & 1     & 2     & 4    & 8    & 16   \\
\cmidrule(lr){1-6}
    %Linear probe CLIP & 36.7 & 47.6 & 57.2 & 65.0 & 71.1 \\
    %          CoOp & 59.6 & 62.3 & 66.8 & 69.9 & 73.4 \\
    %  CLIP-Adapter & 62.7 & 65.5 & 68.6 & 71.3 & 74.4 \\
    %       ProGrad & 62.6 & 64.9 & 68.5 & 71.4 & 73.9 \\
    %   Tip-Adapter & 62.3 & 64.6 & 66.5 & 68.5 & 70.3 \\
    % Tip-Adapter-F & 64.6 & 66.7 & 69.7 & 72.4 & 75.8 \\
              PLOT & 65.5 & \textbf{68.6} & \textbf{71.2} & 73.5 & 76.2 \\
\rowcolor[gray]{.9}
%               RTOS & \underline{65.5} & 67.4 & 70.3 & 72.7 & 75.8 \\ 
% \rowcolor[gray]{.9}
   Ours & \textbf{66.1} & 68.2 & 71.1 & \textbf{73.6} & \textbf{76.6} \\
\bottomrule[1pt]
\end{tabular}
}
\vspace{-1pt}
\caption{\textbf{Comparison with previous few-shot methods.} Average accuracy of 11 datasets. 
\vspace{-5mm}}
\label{tab:r4_major4_comparison_on_fewshot}
\end{center}
\end{table}

% \begin{table*}[h]
% \begin{center}
% \begin{tabular}{lllllll}
% \hline
% Methods          & Backbone & Training Cost & GFLOPs & Params  & Infer. Speed & GPU Memory \\ \hline
% Zero-shot CLIP   & RN50     & 0             & 6.14   & 39.34M  & 11.85ms      & 1648MiB    \\
% CoOp             & RN50     & 880min        & 6.14   & 39.34M  & 11.85ms      & 1648MiB    \\
% Synthetic        & RN50     & -             & 6.14   & 39.34M  & 11.85ms      & 1648MiB    \\
% CLIP-Adapter     & RN50     & 50min         & 6.14   & 39.87M  & 12.00ms      & 1650MiB    \\
% Tip-Adapter-F    & RN50     & 5min          & 6.17   & 71.72M  & 12.06ms      & 1776MiB    \\
% PLOT             & RN50     & -             & 9.31   & 92.22M  & 29.59ms      & 2908MiB    \\
% Ours             & RN50     & 5min          & 6.32   & 53.10M  & 12.77ms      & 1702MiB    \\ \hline
% \end{tabular}
% \end{center}
%     \caption{
%     Comparison of time efficiency for different methods on 16-shot ImageNet.
%     All experiments are tested with batch size 1 on a single NVIDIA Tesla V100 GPU.
%     Among these metrics, excluding the Training Cost, none account for the text encoder's forward propagation process. 
%     For example, during the inference stage of CoOp, only the extracted text features are utilized as classification weights.
%     }
%     \label{tab:r4_major4_polt}
% \end{table*}

\review{Minor. 1}{Typo error in Eq.~5.}
Thanks. We will correct it in our revision.
%We sincerely apologize for any typo errors. We will thoroughly review and rectify any such mistakes present in the article.
%The correct expression is
%\begin{equation*}
%    \mathcal{P}_{tar} = \frac{
%    \exp( \cos(\mathcal{P}_{anc}, \mathcal{R}) / \tau' )
%    }{
%    \sum_{i=1}^{C_{tar}} \exp( \cos(\mathcal{P}_{anc}, \mathcal{R}_{i}) / \tau' )
%    } ,
%\end{equation*}
%where image-target relation $\mathcal{P}_{tar} \in \mathbb{R}^{C_{tar}}$.

\review{Minor. 2}{$\mathcal{F}$ in Eq.8.}
The symbol $\mathcal{F}$ in Equation 8 owns the same meaning as in Equation 3 which is explained in Lines 153-155. We will clarify this further.

\review{Minor. 3}{Anchor space in line 173.}
%We sincerely apologize for the inadequacy of our expression. Our intended message is that we compute the similarity between image features and anchors' features in relation to target class features. We will adjust our phrasing to clarify any confusion that arose, and we deeply regret any complications this might have introduced.
% \textcolor{red}{NOT CLEARLY STATED YET}
Sorry for this confusion. We want to express the meaning that we compute the similarity between the test image and anchors, as well as the similarity between the target categories and anchors. We will modify this statement in our revision.

==> rebuttal/4r1-LDc8.tex <==
We apologize for the lack of clarity in our initial description, which raised concerns from the reviewers. 
We provide further clarification in the following explanation.

\textbf{Q1: Concern about anchors.}

1. About learning of anchors.
In the context of a few-shot setting, our approach involves not directly learning discrete anchor words, but rather learning through anchor embeddings $\in \mathbb{R}^{D}$($D=512$ for ViT-B/16 CLIP). 
These anchor embeddings are initialized randomly and allowed to be learned freely. 
The resulting anchor embeddings can capture semantic information beyond the scope of the existing vocabulary. 
The space in which these anchor embeddings reside is continuous, whereas the categories' names belong to a discrete vocabulary set~(i.e. WordNet). 
Given the continuous nature of the anchor embedding space, its updating mechanism aligns with that of the parameters within the network. 
Furthermore, in the context of a few-shot setting, the term "anchor pool" could lead to confusion, as it might suggest a collection with discrete attributes. 
Since anchor embeddings are learned in the continuous space~$\mathbb{R}^{D}$, we have chosen not to employ the term ``anchor pool" in our paper. 

2. \red{Rationality of learning anchors from target categories data.}
% It is weird to learning the anchors from the few-shot training dataset itself, since these classes are used to learn the classifier. How do they support themselves? 
% 这个问题的意思是不是，借助anchors进行更好的分类，为什么这些anchors可以从target categories数据中学到。这里暂时还没有想出来怎么写。
% CoOp学习到的content prompt可以归因于对图片content信息的期望，但是的确这里有点迷惑。
% 想了个解释，不确定是否靠谱：人们认识若干新事物的时候，一个有效的方式是与已认识的事物进行对比，寻找新事物和旧事物的区别与关联。在这个过程中，人们会思考采用何种事物作为参照物能够对新事物进行更好的区分（显然，人们不可能选择与这些新事物毫无关联的事物作为参照物），我们认为这个思考的过程与anchor的更新是一致的。
% 但是对于这个解释，是不是不该用新旧事物作为比喻，因为对于CLIP来说，应该都属于旧事物。（对于anchor-image relation， relation matrix而言，这个relation matrix对target class直接使用text encoder提取特征，因此这个过程貌似也把target classes认为成了旧事物，如果这个target classes 的feature是直接从image feature得到的话，这个解释就比较合理了？）
This is a thought-provoking question. When people encounter various new concepts, an effective approach is to juxtapose them with familiar ones, seeking to identify distinctions and connections between the novel and the known. During this process, individuals ponder over which references could best differentiate and characterize the new elements (clearly, references with no apparent relevance to these new concepts would not be chosen). We believe that this thought process aligns with the updating of anchors.

As individuals engage in this comparison and connection process, they essentially create mental "anchors" that help them navigate the conceptual landscape. Just as anchors in our approach are updated to better align with target domain data, these cognitive anchors shift and adapt as more information is gained. This dynamic adjustment of mental references is akin to the anchor updating mechanism in our model.

In essence, the process of selecting and adjusting cognitive anchors serves as a analog to the anchor update in our model. This parallel provides a deeper understanding of how our approach mirrors cognitive mechanisms that humans naturally employ when encountering and integrating new information.

3. About supervision.
% Or do we learn the anchors from other classes? Does this make the comparison unfair?
% 这个we用的，哈哈。
Just like previous methods, we utilized the same data and labels for supervision, without introducing any additional forms of guidance.

\textbf{Q2: Details of RTM.}

The inputs of RTM are 
the test image feature $F_{test} \in \mathbb{R} ^ {1 \times  D}$, 
the anchor L2 normalized features $\mathcal{F}_{anc} \in \mathbb{R}^{C_{anc} \times D}$ 
and anchor-target relation matrix $\mathcal{R} \in \mathbb{R}^{ C_{tar} \times C_{anc} }$.
When using ViT-B/16 as the image encoder for training CLIP on ImageNet, $D=512$ and $C_{tar}=1000$.

Let $Q=F_{test}, K=\mathcal{F}_{anc}$ and $V=\mathcal{R}^T$.
The computational process of RTM is as follows:

\begin{align*}
Q',K',V'&=\text{LN}_{qk}(Q), \text{LN}_{qk}(K), \text{LN}_v(V) \\
X &= Q + \text{Attn}(Q', K', V') \\
X &= X + \text{MLP}(\text{LN}_2(X)) \\ 
X &= \text{Proj}(X) .
\end{align*}

We manually calculated the parameter counts of various modules in the model and performed a double-check using the third-party library fvcore.
We report the parameters' details in Tab.~\ref{params_of_rtm}.

\begin{table*}
\begin{center}
\begin{tabular}{lllc}
\hline
module & pytorch                                    & params\_name    & params       \\ \hline
LN$_{qk}$ & nn.LayerNorm(512)                          & weight          & 512          \\
       &                                            & bias            & 512          \\
LN$_v$  & nn.LayerNorm(1000)                         & weight          & 1000         \\
       &                                            & bias            & 1000         \\
Attn   & nn.MultiheadAttention(512, 8, v\_dim=1000) & q\_proj\_weight & (512, 512)   \\
       &                                            & k\_proj\_weight & (512, 512)   \\
       &                                            & v\_proj\_weight & (512, 1000)  \\
       &                                            & in\_proj\_bias  & 3x512        \\
       &                                            & out\_proj       & 512x512      \\
LN$_2$  & nn.LayerNorm(512)                          & weight          & 512          \\
       &                                            & bias            & 512          \\
MLP    & nn.Linear(512, 4x512)                      & weight          & (4x512, 512) \\
       &                                            & bias            & 4x512        \\
       & GELU()                                     & nan             & 0            \\
       & nn.Linear(4x512, 512)                      & weight          & (512, 4x512) \\
       &                                            & bias            & 512          \\
Proj   & nn.Linear(512, 1000)                       & weight          & (1000, 512)  \\
       &                                            & bias            & (1000,)      \\ \hline
Total  &                                            &                 & 3.9M         \\ \hline
\end{tabular}
\end{center}
\caption{Parameters of RTM.}
\label{params_of_rtm}
\end{table*}

\textbf{Q3: Comparison with PLOT.}
% The improvement beyond PLOT is not very significant.
% 相对于第一次的表述It seems to achieve similar or even better results than this submission. 貌似审稿人的语气稍微还行？
% 就是不太确定这句话要不要回。
PLOT is an outstanding piece of research.
Our approach for performance enhancement is orthogonal to that of PLOT, thereby suggesting the potential for achieving improved performance through their ensemble.

Thank you very much for the aforementioned questions. 
We hope our response has addressed the reviewer's concerns. 
Should the reviewer have any additional questions or concerns, we are more than willing to provide further clarification.


-------------------------------------

Thanks for the reviewer’s valuable feedback. Hope our detailed explanations below would clarify your concerns.

\textbf{Q1: Details about learning anchors.}

%- The related description about learning the anchors includes Lines 134-152. 
%In line 149, the $\boldsymbol{s}_{anc, j}$ denotes word embedding of the $j$-th anchors name $\mathrm{s}_{j} \in \mathbb{R}^{D}$($D=512$ for ViT-B/16 CLIP), which is the parameter we need to learn. 
%Let $\mathcal{P}_{final} \in \mathbb{R}^{N C_{tar} \times C_{tar}}$ denote the final prediction, $L_{GT} \in \{0, 1\}^{N C_{tar} \times C_{tar}}$ denotes the one-hot labels of total $N C_{tar}$ training images, where $N$ is the number of shots. 
%The loss function $\mathcal{L} = \mathcal{L}_{CE}(\mathcal{P}_{final}, L_{GT})$.
Sorry for this confusion. In our original version, we explain what the anchor is in Line 134-152. The equations (3-5) explain the idea of utilizing anchors to support classification prediction. We provide more details below and will revise our paper accordingly.

% The equation explaining how to learn the anchors is xxx. 

- To clarify the reviewer’s concern, we first introduce how to use anchors for prediction. We deal with the few-shot classification task, where we aim to attach a label to the input image. That is, we need to know the relationships between the input image and the target classes to make predictions. In our paper, we first build an anchor-target matrix, which depicts the similarities between the anchors and target classes. Then, we compute the image-anchor vector, which denotes the similarities between the input image and the anchors. Finally, a straightforward way to achieve the  image-target relationships is to multiply the image-anchor vector and the anchor-target matrix. In our paper, we design a transformer architecture (*i.e.,* RTM module) to obtain the image-target relationships based on the image-anchor similarities and anchor-target similarities. Details about how RTM realizes this can be found in the following answers to Q2. 

- We want anchors to represent open semantics. Thus, in our design, we fix the prompt (or context) and make the class token learnable in the text input, *e.g.,* “A photo of [class]” where the “[class]” token is learnable. Each learnable class token corresponds to an anchor. We may achieve the anchor representation by forwarding the corresponding text input through the text encoder of CLIP. Then, the above-mentioned image-anchor vector and the anchor-target matrix can be readily calculated. 

- For the learning of anchors, *i.e.,* the learning of different class tokens, we just utilize the data from the target task. We don’t use any additional data to learn the anchors. Our experiment setting is identical to [11]. Thus, our comparisons with previous CLIP-based few-shot learning methods are fair.

- For the reasons why the few-shot images are possible to support the anchor learning, we speculate it is because we utilize the knowledge from CLIP. As we fix the CLIP encoders, the embedding of anchor has high probability to represent a semantic. The few-shot training data just needs to “select” the most useful semantics to facilitate the classification. Due to the data limit, the “selection” may not be optimal but it should be better than the randomly initialized anchors whose performance is already comparable to the CLIP zero-shot baseline (see Tab. 1 of the paper).  

- For ``anchor pool", we don’t utilize this saying in our paper. It is used by Reviewer JQvo’s comment. We speculate that the reviewer is referring to how the anchors are chosen. We have answered this question in the above statement. 

- We are quite certain that our results are correct and our comparisons are fair. We also provide our code. If interested in more details of our paper, the reviewer may check our code.

\textbf{Q2: The amount of parameters in the RTM module.}

- First, we provide more details about the architecture of RTM module. Let $F_{test} \in \mathbb{R} ^ {1 \times  D}$ denotes the test image feature, $\mathcal{F}_{anc} \in \mathbb{R}^{C_{anc} \times D}$ denotes the anchor L2 normalized features, and $\mathcal{R} \in \mathbb{R}^{ C_{tar} \times C_{anc} }$ denotes anchor-target relation matrix.
When using ViT-B/16 as the image encoder for training CLIP on ImageNet, $D=512$ and $C_{tar}=1000$.
Let $Q=F_{test}, K=\mathcal{F}_{anc}$ and $V=\mathcal{R}^T$.
The computational process of RTM is as follows:
\begin{align*}
Q',K',V'&=\text{LN}_{qk}(Q), \text{LN}_{qk}(K), \text{LN}_v(V) \\
X &= Q + \text{Attn}(Q', K', V') \\
X &= X + \text{MLP}(\text{LN}_2(X)) \\ 
X &= \text{Proj}(X) .
\end{align*}

- We provide the details of how to compute the amount of parameters in RTM in the following table. 

\textbf{Q3: The improvement beyond PLOT is not very significant.}

We will cite and make more comparisons with PLOT in our revised version. Our method is orthogonal to PLOT and can be combined with PLOT to improve the few-shot learning results further, as shown in the table below. Due to the high GPU memory consumption of training PLOT, we only report results on eight out of eleven datasets. We will provide results for the remaining three datasets in the future.

%We report the results by ensembling PLOT and our method. We directly calculate the arithmetic average of probabilities (not logits) from both methods to obtain the ensemble result. Due to the high GPU memory requirements for training the PLOT network, our current hardware can only support model training on eight out of the eleven datasets. We will provide results for the remaining three datasets in the future.

\begin{table}[]
\begin{tabular}{lccccc}
\toprule
 & 1 & 2 & 4 & 8 & 16 \\
\midrule
PLOT      & 65.6 & 69.5 & 72.6 & 76.1 & 77.9 \\
Ours      & 65.6 & 68.1 & 71.7 & 74.6 & 78.2 \\
PLOT+Ours & 67.2 & 70.9 & 73.5 & 76.6 & 78.8 \\
% SEARCH  & 68.2 & 72.0 & 74.4 & 77.1 & 79.4 \\
\bottomrule
\end{tabular}
\caption{Average results on 8 datasets: eurosat, caltech101, stanford\_cars, oxford\_pets, oxford\_flowers, dtd, ucf101, fgvc.}
\end{table}

==> rebuttal/5-Record.tex <==
\subsection{Method}


\begin{table}[h]
\begin{center}
\begin{tabular}{llll}
\hline
     & ZS-CLIP & CoOp & RTOS-C \\ \hline
mIoU & 18.6           & 19.6 & 21.5   \\ \hline
\end{tabular}
\end{center}
\caption{
\textbf{Semantic Segmentation Performance on VOC2012 with mIoU Metric.} 
We evaluated the segmentation performance on the VOC2012 dataset using a subset of 65 images. This subset was carefully selected to ensure that each class is represented in approximately 4 images. These images were used to form the training set, while the VOC2012 validation set was employed for validation purposes. We employed an RN50 backbone with a configuration that involved resizing the shorter side of the images to 320 pixels, aiming for rapid verification of the method's effectiveness. To achieve semantic segmentation, we modified the Global Attention Pooling of the final layer in the RN50 CLIP model to calculate similarity on a per-patch, following the paradigm of MaskCLIP.
}
\end{table}

\begin{table*}[h]
  \centering
  \begin{subtable}[b]{0.48\linewidth}
    \centering
\begin{tabular}{llllll}
\toprule
 & 1 & 2 & 4 & 8 & 16 \\
\midrule
eurosat & 62.3 & 66.4 & 76.3 & 78.4 & 83.0 \\
caltech101 & 89.4 & 89.8 & 90.1 & 90.9 & 93.0 \\
imagenet & 60.7 & 61.0 & 61.8 & 62.8 & 63.8 \\
stanford\_cars & 57.4 & 60.0 & 62.2 & 67.0 & 73.2 \\
food101 & 77.6 & 77.8 & 78.1 & 78.6 & 79.0 \\
oxford\_pets & 86.0 & 86.5 & 87.5 & 88.1 & 88.8 \\
oxford\_flowers & 76.5 & 79.7 & 87.0 & 90.3 & 94.0 \\
dtd & 49.9 & 53.4 & 58.7 & 61.8 & 65.9 \\
sun397 & 61.4 & 63.8 & 66.7 & 67.5 & 69.8 \\
ucf101 & 65.4 & 67.5 & 70.6 & 74.7 & 78.3 \\
fgvc & 20.6 & 22.6 & 23.6 & 28.0 & 32.8 \\
average & 64.3 & 66.2 & 69.3 & 71.6 & 74.7 \\
\bottomrule
\end{tabular}
    \caption{Unified context prompt}
    \label{subtableA}
  \end{subtable}
  \hfill
  \begin{subtable}[b]{0.48\linewidth}
    \centering
\begin{tabular}{llllll}
\toprule
 & 1 & 2 & 4 & 8 & 16 \\
\midrule
eurosat & 63.5 & 68.6 & 75.7 & 76.6 & 82.9 \\
caltech101 & 89.2 & 89.2 & 90.6 & 90.8 & 92.5 \\
imagenet & 60.8 & 60.9 & 61.8 & 62.7 & 63.7 \\
stanford\_cars & 57.2 & 59.3 & 61.8 & 65.8 & 73.0 \\
food101 & 77.4 & 77.7 & 78.0 & 78.5 & 78.9 \\
oxford\_pets & 86.2 & 86.5 & 87.1 & 87.8 & 88.4 \\
oxford\_flowers & 76.3 & 78.9 & 86.9 & 90.0 & 93.5 \\
dtd & 48.2 & 53.2 & 57.0 & 61.2 & 65.8 \\
sun397 & 61.4 & 63.3 & 66.2 & 67.4 & 69.8 \\
ucf101 & 64.7 & 67.1 & 69.9 & 73.2 & 76.9 \\
fgvc & 20.9 & 22.0 & 24.4 & 27.9 & 35.8 \\
average & 64.1 & 66.1 & 69.0 & 71.1 & 74.7 \\
\bottomrule
\end{tabular}
    \caption{Class-specific context prompt}
    \label{subtableB}
  \end{subtable}
  \caption{Results of simultaneous training of context prompts and class name embeddings.}
\end{table*}

\begin{table*}[h]
\begin{center}
\begin{tabular}{lllllll}
\hline
Methods        & Backbone & Training Cost & GFLOPs & Params  & Infer. Speed & GPU Memory \\ \hline
Zero-shot CLIP   & RN50     & 0             & 6.14   & 39.34M  & 11.85ms      & 1648MiB    \\
CoOp             & RN50     & 880min        & 6.14   & 39.34M  & 11.85ms      & 1648MiB    \\
Synthetic        & RN50     & -             & 6.14   & 39.34M  & 11.85ms      & 1648MiB    \\
CLIP-Adapter     & RN50     & 50min         & 6.14   & 39.87M  & 12.00ms      & 1650MiB    \\
Tip-Adapter-F    & RN50     & 5min          & 6.17   & 71.72M  & 12.06ms      & 1776MiB    \\
PLOT             & RN50     & -             & 9.31   & 92.22M  & 29.59ms      & 2908MiB    \\
RTOS             & RN50     & 5min          & 6.32   & 53.10M  & 12.77ms      & 1702MiB    \\ \hline
Zero-shot CLIP   & ViT-B16  & 0             & 17.58  & 86.70M  & 10.40ms      & 1710MiB    \\
CoOp             & ViT-B16  & 1724min       & 17.58  & 86.70M  & 10.40ms      & 1710MiB    \\
Synthetic        & ViT-B16  & -             & 17.58  & 86.70M  & 10.40ms      & 1710MiB    \\
CLIP-Adapter     & ViT-B16  & 73min         & 17.58  & 86.84M  & 10.66ms      & 1710MiB    \\
Tip-Adapter      & ViT-B16  & 7min          & 17.61  & 110.90M & 10.69ms      & 1804MiB    \\
Maple            & ViT-B16  & 66min         & 17.77  & 86.72M  & 11.08ms      & 1710MiB    \\
RTOS             & ViT-B16  & 8min          & 17.65  & 90.74M  & 11.23ms      & 1716MiB    \\ \hline
\end{tabular}
\end{center}
    \caption{
    Comparison of time efficiency for different methods on 16-shot ImageNet.
    All experiments are tested with batch size 1 on a single NVIDIA Tesla V100 GPU.
    Among these metrics, excluding the Training Cost, none account for the text encoder's forward propagation process. 
    For example, during the inference stage of CoOp, only the extracted text features are utilized as classification weights.
    }
\end{table*}

\begin{table*}[h]
    \centering
\begin{center}
\begin{tabular}{lccccccccccc}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{\raisebox{-7ex}{Anchors}}} & \multicolumn{10}{c}{Target Dataset} \\ \cmidrule(lr){2-12}
 & \rotatebox{65}{ImageNet} & \rotatebox{65}{SUN397} & \rotatebox{65}{EuroSAT} & \rotatebox{65}{UCF101} & \rotatebox{65}{Food101} & \rotatebox{65}{OxfordPets} & \rotatebox{65}{StandfordCars} & \rotatebox{65}{Flowers102} & \rotatebox{65}{FGVCAircraft} & \rotatebox{65}{Caltech101} & \rotatebox{65}{DTD} \\
\midrule
ImageNet & 60.3 & 58.7 & 36.1 & 61.7 & 77.4 & 85.4 & 55.8 & 66.0 & 16.6 & 86.6 & 43.1 \\
SUN397 & 33.1 & 58.9 & 36.1 & 61.7 & 77.4 & 85.5 & 55.8 & 66.0 & 16.6 & 87.1 & 43.2 \\
EuroSAT & 60.3 & 58.9 & 36.2 & 61.9 & 77.4 & 85.8 & 55.8 & 66.1 & 17.0 & 85.9 & 43.0 \\
UCF101 & 59.6 & 58.8 & 36.2 & 61.9 & 77.4 & 85.5 & 55.8 & 66.0 & 16.6 & 86.5 & 42.9 \\
Food101 & 56.9 & 58.9 & 36.2 & 61.9 & 77.3 & 85.6 & 55.8 & 65.9 & 17.0 & 86.1 & 43.0 \\
OxfordPets & 60.3 & 58.8 & 37.2 & 61.9 & 77.4 & 85.8 & 55.7 & 66.0 & 17.0 & 85.9 & 43.2 \\
StandfordCars & 30.3 & 58.8 & 36.4 & 62.0 & 77.4 & 85.8 & 55.8 & 66.0 & 17.2 & 85.9 & 42.9 \\
Flowers102 & 46.2 & 58.9 & 36.2 & 61.8 & 77.4 & 85.8 & 55.8 & 66.1 & 16.8 & 86.1 & 42.9 \\
FGVCAircraft & 30.2 & 58.9 & 39.3 & 61.8 & 77.4 & 85.8 & 55.8 & 66.1 & 17.0 & 85.9 & 43.3 \\
Caltech101 & 60.3 & 58.8 & 37.2 & 61.8 & 77.4 & 85.5 & 55.8 & 66.1 & 16.5 & 85.8 & 43.0 \\
DTD & 60.3 & 58.8 & 37.7 & 61.8 & 77.4 & 85.5 & 55.8 & 66.1 & 16.7 & 87.5 & 42.8 \\
ImageNet21k & 30.2 & 58.6 & 35.9 & 60.3 & 77.4 & 83.3 & 55.7 & 65.9 & 16.7 & 86.8 & 43.1 \\
Zero-shot CLIP & 60.3 & 58.9 & 36.2 & 61.9 & 77.3 & 85.8 & 55.8 & 66.1 & 17.0 & 85.8 & 42.8 \\
\bottomrule
\end{tabular}
\end{center}
\vspace{-3mm}
    \caption{Zero-shot results using 11 datasets as anchor datasets for each other.}
\vspace{-3mm}
\end{table*}

\begin{table*}[h]
\begin{center}
\begin{tabular}{l|cccccccc}
\hline
  & 0        & 1           & 2           & 3           & 4           & 5       & 6           & 7            \\ \hline
0 & foregone & www         & lassa       & mugil       & msh         & choler  & syndic      & tipple       \\
1 & weal     & chyle       & canful      & jumbojet    & uxoriously  & bennett & cer         & plage        \\
2 & sestet   & tax         & program     & lld         & querier     & footage & ton         & joe\_louis   \\
3 & bit      & corday      & coreid      & duds        & gigo        & gabor   & lizard      & succinctness \\
4 & garroter & rodent      & inscriptive & andrew      & bit         & jut     & introitus   & bibliotics   \\
5 & mitchum  & unabashedly & goodish     & retrorocket & somberness  & jut     & perusal     & degrader     \\
6 & aneurism & revery      & ddc         & saran       & hodur       & also    & gish        & potential    \\
7 & one\_c   & utterly     & sweet\_cup  & at\_least   & rynchops    & l       & ido         & deviant      \\
8 & phot     & pithiness   & emmer       & eskimo\_dog & coffee\_cup & weasel  & monaul      & self-torment \\
9 & certain  & aneurism    & annals      & zee         & sooth       & orono   & incessantly & phot         \\ \hline
\end{tabular}
\end{center}
\caption{Closest words in WordNet to the 80 anchors learned from Caltech101 16-shot.}
\end{table*}

==> section/Abstract-v0.tex <==
\begin{abstract}
  Contrastive Vision-Language Pre-training (CLIP) has achieved impressive zero-shot performance on downstream tasks by learning visual representations from image-text pairs. 
  To improve its few-shot capabilities, Tip-Adapter introduces a feature retrieval adapter. However, as the number of retrieval features increases with the number of shots, the adapter becomes heavier and less efficient.
  ICR-Transposer is proposed in this paper to address the data limitation problem in classification tasks. 
  By introducing an auxiliary set of categories, ICR-Transposer models the relationship between the auxiliary and target category sets using inter-class relation(ICR) modeling. 
  This modeling technique allows ICR-Transposer to transform the probabilities of image classification from the auxiliary category set to the target category set using probability transformation. 
  ICR-Transposer not only improves the performance of zero-shot classification in a training-free and data-free manner, but also performs comparably to those training-required approaches in few-shot setting. 
  To demonstrate the effectiveness of ICR-Transposer, experiments of zero-shot and few-shot classification are conducted on 11 datasets. 
  The results show that ICR-Transposer outperforms existing state-of-the-art methods in both zero-shot and few-shot classification settings.
  Code will be released soon. 
\end{abstract}

==> section/Abstract-v1.tex <==
\begin{abstract}
  Contrastive Vision-Language Pre-training~(CLIP) achieves impressive zero-shot performance on downstream tasks.
  %by learning visual representations from image-text pairs. 
  To enhance the downstream classification capabilities of CLIP, previous approaches typically utilize vision features from additional training images, which are usually hard to collect in fain-grained circumstances.
  %However, CLIP itself already models the relationships between different semantic concepts, and exploring how to leverage these semantic associations remains unexplored.
  The linguistic data, on the contrary, is easy to obtain while possessing rich concept correlations for the adaptation of different classification tasks.
  Inspired, we propose Inter-Class Relation~(ICR) Transposer to transpose knowledge from a set of anchor categories to target categories with a class-shifting matrix,
  thereby achieving efficient classification adaptation with solely linguistic data.
  %\textit{ICR-Transposer} is proposed in this paper to leverage the semantic associations built by CLIP in classification tasks. 
  Specifically, ICR Transposer generates a class-shifting matrix by performing an inner product between anchor class embeddings and target class embeddings, and then utilizes a probability transposer to transfer anchor probabilities to target probabilities.
  % 1. How to represent/obtain the anchor classes
  % 2. How to transform information, (such as, generate a class-shifting matrix by inner-product between anchor class embeddings and target class embeddings)
  % How to obtain the target probability
% (1) time partition
% (2) title -> ab -> intro 。摘要是题目的延续，intro是摘要的延续
% (3) background -> existing methods/challenge/problem -> our methods(how to solve the mentioned problem) -> experiment。这是一个基本的模板，写的牛逼了可以不按照这个，但是按照这个来总没错。
% （4）写之前整个故事线要想好。challenge/problem是什么，要解决的东西是什么（这个东西想不清楚，你的文章就没有价值）。然后为了解决这个问题，你的方法是怎么做的，这个过程中尽量点题，提炼核心contribution
% (5) abstract里面每句话都很关键，尽量不说废话，例如ICR-Transposer not only improves the performance of zero-shot classification in a training-free and data-free manner, but also performs comparably to those training-required approaches in few-shot setting. 这么长的一句话就想表达zs和fs指标都提高了，废话太多，而且跟下面讲实验的话重复
% (6) 少用this, it, its, 指代不明，不够准确
% (7) 长句子目的在前，做法在后。尽量让读者在读后面部分的时候就知道你要干啥。例如为了XX，我们干了A，干了B，干了C。而不是我们干了A，干了B，干了C，是为了XX。
%（8）每句话都要有目的性。
%By introducing extra prototypes, ICR-Transposer models the relationship between target categories and extra prototypes using \textbf{I}nter-\textbf{C}lass \textbf{R}elation(ICR) modeling. 
 %This modeling technique allows \textit{ICR-Transposer} to transpose the probabilities of image classification from extra prototypes to the target categories.
 %这两句话，一点作用/价值/效益都没有体现，单纯的说我做了什么，我做了什么。这种句子在method里面可以，但是在摘要里面不行。摘要里面讲方法的句子要跟你前面的内容结合，例如怎么样解决的前面提出的问题，怎么样实现了你前面设定的目标。
% （9）文章中不要提问，有啥直接说啥。intro里面这种写法看起来就很奇怪。
% （10）尽量少用被动时态
%
%
  %By introducing extra prototypes, ICR-Transposer models the relationship between target categories and extra prototypes using \textbf{I}nter-\textbf{C}lass \textbf{R}elation(ICR) modeling. 
  %This modeling technique allows \textit{ICR-Transposer} to transpose the probabilities of image classification from extra prototypes to the target categories. 
  %\textit{ICR-Transposer} not only improves the performance of zero-shot classification in a training-free and data-free manner, but also performs comparably to those training-required approaches in few-shot setting. 
  We conduct extensive experiments on 11 classification datasets.
  %To demonstrate the effectiveness of \textit{ICR-Transposer}, experiments of zero-shot and few-shot classification are conducted on 11 datasets. 
  The results show that \textit{ICR-Transposer} outperforms existing state-of-the-art methods in both zero-shot and few-shot classification settings. 
  Code is released at \href{https://anonymous.4open.science/r/ICR-Transposer}{https://anonymous.4open.science/r/ICR-Transposer}.
\end{abstract}

==> section/Introduction.tex <==
\section{Introduction}

In recent years, large vision-language pre-trained models(VLM), \textit{e.g.} CLIP~\cite{radford2021learning}, ALIGN~\cite{jia2021scaling}, ALEBF~\cite{li2021align}, VLMO~\cite{bao2022vlmo}, LOUPE~\cite{li2022fine}, have achieved remarkable performance on downstream vision tasks, such as classification~\cite{zhang2022tip,zhou2022learning,guo2022texts,lin2023multimodality}, segmentation~\cite{xu2023open,xu2023learning,luo2022segclip,liang2022open}, detection~\cite{yao2022detclip,zhang2022glipv2,minderer2022simple,feng2022promptdet} and image generation~\cite{nichol2021glide,ramesh2022hierarchical,saharia2022photorealistic,seale2023continual}. 
VLM usually consist of data encoders and utilize image-text contrastive loss~\cite{radford2021learning} to align the embedding of images and texts into a shared space. 
When adapting pre-trained models to classification tasks in specific scenarios lacking annotated data, fine-tuning the entire model tends to be ineffective due to its high complexity.
Prompt tuning~\cite{zhou2022learning,zhou2022conditional} and adapter~\cite{zhang2022tip,gao2021clip} have emerged as representative parameter-efficient learning paradigms that adapt VLM to downstream tasks.

Albeit considerable achievements have been made, existing prompt tuning and adapter methods have primarily focused on extracting and utilizing features from CLIP to enhance performance. 
For example, CoOp~\cite{zhou2022learning} learns from annotated images to extract broader textual features. 
Tip-Adapter~\cite{zhang2022tip} improves few-shot performance by using existing data as adapter parameters and performing feature retrieval. 
TaI-DPT~\cite{guo2022texts} trains prompt using text samples that contain classes specific to the target domain. 
He et al. \cite{he2022synthetic} fine-tune the CLIP classifier using synthetic images as training samples.
In summary, these methods primarily concentrate on extracting and leveraging features from CLIP to improve performance. 
Additional, zero-shot methods by CLIP typically extract text features for a set of class names and select the nearest one to the image feature as the classification result.
One noteworthy fact is that CLIP adeptly models semantic associations by means of contrastive learning between image and text pairs. 
However, the exploration of how to leverage these semantic associations to enhance CLIP's performance in downstream tasks remains unexplored. In this paper, we semantic relationships constructed by CLIP to improve CLIP's classification.

% Consequently, we raise two pivotal questions: 
% \quad 1. \textit{Can the semantic relationships constructed by CLIP effectively improve its performance in downstream tasks?} 
% \quad 2. \textit{How can we optimize the utilization of the semantic associations built by CLIP?}


% \begin{figure}
% \begin{center}
% \includegraphics[width=0.5\linewidth]{figure/class_relation.pdf}
% \end{center}
%    \vspace{-4mm}
% \caption{Transforming probabilities from extra prototypes to target classes using inter-class relation.}
% \vspace{-7mm}
% \label{fig:class_relation}
% \end{figure}

\begin{wrapfigure}{r}{0.5\textwidth}
  \centering
  \includegraphics[width=1.0\linewidth]{figure/class_relation.pdf}
  \vspace{-4mm}
\caption{Transforming probabilities from extra prototypes to target classes using inter-class relation.}
\vspace{-7mm}
\label{fig:class_relation}
\end{wrapfigure}



As shown in Fig.~\ref{fig:class_relation}, when we know the probability of an image belonging to anchor categories (blue), but not to target categories (green), we can use the class-shifting matrix (red) to transfer the probability from anchor categories to target categories.
Specifically, when we encounter the depicted animal in Fig.~\ref{fig:class_relation}, we recognize its resemblance to a cat and a kangaroo but remain uncertain about its specific classification, whether it is a tiger-cat, chinchilla, anteater, or lemur. However, with access to information about the inter-class relations, depicted by the red lines in Fig.~\ref{fig:class_relation}, between these four animals (tiger-cat, chinchilla, anteater, lemur) and other animals like tiger, cat, kangaroo, and pig, we can make a reasonable inference that the animal in Fig.~\ref{fig:class_relation} is most likely a chinchilla.
% Specifically, if we only know that the animal in the image is likely a terrier, but do not know if it is a dog, if there is a concept that the terrier is a type of dog, we can easily infer that the animal in the image is likely a dog. In cases where labeled data is limited, knowledge of inter-class relations can be leveraged to improve performance.

In this paper, we propose a method called \textbf{I}nter-\textbf{C}lass \textbf{R}elation \textbf{Transposer} (ICR-Transposer) to enhance the classification performance of CLIP. To transform the probability of a given image belonging to anchor categories to the probability of it belonging to target categories, we introduce anchor categories and leverage the text encoder of CLIP to model the inter-class relation between anchor categories and target categories.
Furthermore, in a few-shot setting, updating anchor categories with a small amount of data empowers the model to enhance the quality of the additional prototypes. Our ICR-Transposer is also compatible with multiple modalities of data, further improving model performance. By working only with few-shot image data, our approach achieves state-of-the-art performance on 11 datasets.
Our contributions can be summarized as follows:

$\bullet$ We have proposed an idea to enhance the performance of Vision-Language Models by incorporating semantic correlations.

$\bullet$ We introduce ZS-ICR-Transposer and ICR-Transposer, which model inter-class relations to enhance the zero-shot and few-shot performance of CLIP.

$\bullet$ We evaluate ZS-ICR-Transposer and ICR-Transposer on 11 widely-adopted datasets for few-shot classification and conduct extensive ablation studies to demonstrate their stat-of-the-art characteristics.

==> section/Method-v0.tex <==
\section{Method}

\begin{figure*}
\begin{center}
\includegraphics[width=1.0\linewidth]{figure/architecture.pdf}
\end{center}
   \vspace{-3mm}
\caption{\textbf{The Pipeline of ICR-Transposer.} 
\textcolor[rgb]{0.796875, 0.3984375, 0.0}{{(a) Inter-class Relation Modelling}}: Input with the target classes and the auxiliary class, the CLIP text encoder is adopted to extract the target classes features $\boldsymbol{F}_{tgt}$ and the auxiliary classes features $\boldsymbol{F}_{aux}$, which are used to model the inter-class relation $\boldsymbol{R}$ between target classes and auxiliary classes. Where the auxiliary class can either be randomly initialized or designed manually.
\textcolor[rgb]{0.35546875, 0.5546875, 0.1953125}{{(b) Relation-based Classification}}: Input a test image, the CLIP image encoder is adopted to extract the image feature. Next, the probability transposer is applied to convert the image classification probabilities from the auxiliary classes to the target classes. This knowledge obtained from probability transformation is then incorporated with CLIP's pre-trained knowledge, achieving a training-free adaptation.
It should be noted that the "Tuned Parameters" in the figure refer only to the parameters that need to be fine-tuned in the training-required paradigm. However, these parameters can still contribute to improving CLIP's zero-shot performance even without fine-tuning.
}
\vspace{-4mm}
\label{fig:architecture}
\end{figure*}

\subsection{Zero-shot Setting}

\subsubsection{Training-free}

We propose ZS-ICR-Transposer, a training-free adaption method to enhance the zero-shot classification performance of CLIP. 
Our method introduces additional auxiliary classes, which we distinguish from the target classes in the target domain. 

Following~\cite{zhou2022learning}, we define the target classes prompts and the auxiliary classes prompts given to the text encoder as follows:

\begin{equation}
    \boldsymbol{T}_{tgt,i}=[\boldsymbol{v}_1, \boldsymbol{v}_2, \boldsymbol{v}_3, ...,\boldsymbol{v}_M, \boldsymbol{s}_{tgt, i}]
    \label{eq:prompt_target}
\end{equation}

\begin{equation}
    \boldsymbol{T}_{aux,j}=[\boldsymbol{v}_1, \boldsymbol{v}_2, \boldsymbol{v}_3, ...,\boldsymbol{v}_M, \boldsymbol{s}_{aux, j}]
    \label{eq:prompt_auxiliary}
\end{equation}

where $i\in \{1, 2, ..., C_{tgt} \}$ is the target class index, $\boldsymbol{s}_{tgt, i}$ denotes word embedding of the $i$-th target class name $\mathrm{s}_{i}$, $j \in \{1, 2, ..., C_{aux} \}$ is the auxiliary class index, the $\boldsymbol{s}_{aux, j}$ denotes word embedding of the $j$-th auxiliary class name $\mathrm{s}_{j}$ if the auxiliary class was designed manually else randomly initialized vector. For $k\in \{1, 2, ..., M\}$, $\boldsymbol{v}_{k}$ denotes word embedding of the $k$-th word of prompt sentences (\textit{e.g.} $\texttt{"A photo of \{\}."}$).

As shown in Fig.~\ref{fig:architecture}(a), by forwarding the target class prompts $\boldsymbol{T}_{tgt}$ and the auxiliary class prompts $\boldsymbol{T}_{aux}$ to the CLIP text encoder, we can obtain the target class features $\boldsymbol{F}_{tgt} \in \mathbb{R}^{C_{tgt} \times 
 D}$ and the auxiliary class feature $\boldsymbol{F}_{aux} \in \mathbb{R}^{C_{aux} \times D}$. The features of target classes and auxiliary classes are used to build the Inter-class Relation, the Inter-class Relation $\boldsymbol{R} \in \mathbb{R}^{ C_{tgt} \times C_{aux} }$ is defined as:

\begin{equation}
     \boldsymbol{R}_{i,j} = \frac{\exp(\cos(
     \boldsymbol{F}_{tgt, i},\boldsymbol{F}_{aux, j}
     )/\tau)}{
\sum\nolimits_{j=1}^{C_{aux}} \exp(\cos(
     \boldsymbol{F}_{tgt, i},\boldsymbol{F}_{aux, j}
     )/\tau) 
} 
\end{equation}

As shown in Fig.~\ref{fig:architecture}(b), by forwarding the test image $\boldsymbol{I} \in \mathbb{R} ^ {H \times W \times 3}$ to the CLIP image encoder, we can obtain the test image feature $f_{test} \in \mathbb{R} ^ {D}$.
The Probability Transposer is a cross-attention module, which accepts the image feature $f_{test}$ as query, the auxiliary class features $\boldsymbol{F}_{aux}$ as keys, and the Inter-class Relation $\boldsymbol{R}$ as values. The processing of Probability Transposer is defined as:

\begin{equation}
    \rm{logits}_{ICR} = \texttt{CrossAttn}(f_{test}\boldsymbol{W}_{\rm{q}}^T, \boldsymbol{F}_{aux}\boldsymbol{W}_{\rm{k}}^T, \boldsymbol{R})
\end{equation}

where $\boldsymbol{W}_{q} \in \mathbb{R} ^ {D \times D} $ is a eye matrix, $\boldsymbol{W}_{k} \in \mathbb{R} ^ {D \times D} $ is a eye matrix. 

And the output logits are calculated as:

\begin{equation}
    \rm{logits} = \alpha \rm{logits}_{ICR} + f_{test} \boldsymbol{F}_{tgt}^T
\end{equation}


Probability Transposer's prediction, therefore, contains two terms, the former term is transformed by Inter-class Relation, and the latter term preserves the prior knowledge from the CLIP's classifier $\boldsymbol{F}_{tgt}$.

\subsubsection{Training-required}

Based on the influence of manually selecting different auxiliary classes on CLIP's zero-shot performance (which will be further investigated in the ablation study section~\ref{sec:ablation_on_auxiliary_selection}), we have identified the key characteristics that auxiliary classes should possess to enhance CLIP's zero-shot performance:

$\bullet$ Auxiliary classes should not exhibit an excessively high correlation with a single category in the target classes while having a very low correlation with other categories. In the extreme case where the auxiliary class is identical to a target class, it does not contribute to improving CLIP's zero-shot performance. Therefore, any auxiliary class should have associations with the target classes that significantly deviate from a one-hot distribution.

$\bullet$ Auxiliary classes should not exhibit similar correlations with all categories in the target classes. In the extreme case where the auxiliary class has identical similarities with all target classes, it also does not contribute to improving CLIP's zero-shot performance. Therefore, any auxiliary class should have associations with the target classes that significantly deviate from a uniform distribution.

$\bullet$ There should not be target classes with extremely low correlations with any auxiliary class. Such target classes would not benefit from the performance improvements derived from inter-class relations.

At first, we define the probability $\boldsymbol{P} \in \mathbb{R}^{ C_{tgt} \times C_{aux} }$ matrix as follows:

\begin{equation}
     \boldsymbol{P}_{i,j} = \frac{\exp(\cos(
     \boldsymbol{F}_{tgt, i},\boldsymbol{F}_{aux, j}
     )/\tau)}{
\sum\nolimits_{i=1}^{C_{tgt}} \exp(\cos(
     \boldsymbol{F}_{tgt, i},\boldsymbol{F}_{aux, j}
     )/\tau) 
} 
\end{equation}

In order to avoid the collapse of the probability distribution of $j$-th auxiliary belonging to target classes $\boldsymbol{P}_j = \{\boldsymbol{P}_{i,j}\}_{i=1}^{C_{tgt}}$ into a one-hot distribution, we can utilize k-means clustering to group the probability distribution into three clusters $\{\mathcal{C}\}_1^3$. Let $k$ represent the index of the cluster with the highest average value, as $ k = {\rm argmax}_{i} \{ \overline{\mathcal{C}_i} \}_1^3$. 
If the length of cluster $k$ is greater than $1$, the loss is assigned as 0. However, if the length of cluster $k$ is equal to $1$, we generate a probability pseudo-label $\boldsymbol{Q}_j = \{ 0.3\  \text{if}\  t\  \text{in}\  {\text{indices}_{top3}} \  \text{else}\  0.1 / (C_{tgt} - 3)\}_{1}^{C_{tgt}}$ and employ KL divergence as the loss function.

\begin{equation}
    \mathcal{L}_{KE} = 
    \begin{cases}
        0, & \text{if length of cluster } k > 1 \\
        \text{KL}(\boldsymbol{P}_j || \boldsymbol{Q}_j), & \text{if length of cluster } k = 1
    \end{cases} 
\end{equation}


To avert the similarity of the $j$-th auxiliary belonging to closes to a uniform distribution, we incorporate the entropy regularize, vis minimizing:

\begin{equation}
    \mathcal{L}_{EH} = \frac{ \sum -\boldsymbol{P}_j^T\log (\boldsymbol{P}_j) }{C_{aux}}
\end{equation}

To any target classes with extremely low correlations with any auxiliary class, we incorporate the entropy regularize, vis minimizing:

\begin{equation}
    \mathcal{L}_{HE} =  \overline{\boldsymbol{P}_j}^T\log (\overline{\boldsymbol{P}_j}) 
\end{equation}


The Prototypes Prior Loss (PP loss) be defined as:

\begin{equation}
    \mathcal{L}_{PP} =  \mathcal{L}_{KE} + \mathcal{L}_{EH} + \mathcal{L}_{HE}
\end{equation}


\subsection{Few-shot Setting}

ZS-ICR Transposer offers a substantial boost to CLIP by incorporating fresh inter-class relation knowledge, even without access to training data, and its performance can be further refined through optimization using the prior loss. 
Moreover, ICR-Transposer remains compatible with situations that involve training data. In the few-shot scenario, a limited amount of data can aid ICR-Transposer in acquiring superior auxiliary classes, thereby elevating its performance even further. 
ICR-Transposer focuses solely on updating the auxiliary class embeddings (which can be pre-designed or randomly initialized) to learn auxiliary classes that provide significant performance improvements to CLIP. 
With the updates made to ICR-Transposer, it attains state-of-the-art performance on 11 widely adopted datasets. For few-shot setting, we use the standard cross-attention transformer block as Probility Transposer.

The total loss be defined as:

\begin{equation}
    \mathcal{L} =  \mathcal{L}_{cls} + \gamma \mathcal{L}_{PP}
\end{equation}


==> section/Method-v1.tex <==
\section{Method}

\begin{figure*}
\begin{center}
\includegraphics[width=1.0\linewidth]{figure/architecture.pdf}
\end{center}
   \vspace{-3mm}
\caption{\textbf{The Pipeline of ICR-Transposer.} 
\textcolor[rgb]{0.796875, 0.3984375, 0.0}{{(a) Inter-class Relation Modelling}}: Input with target classes and prototypes, the CLIP text encoder is adopted to extract the target classes features $\boldsymbol{F}_{tgt}$ and the prototypes features $\boldsymbol{F}_{pro}$, which are used to model the inter-class relation $\boldsymbol{R}$ between target classes and prototypes. Where the prototypes can either be randomly initialized or designed manually.
\textcolor[rgb]{0.35546875, 0.5546875, 0.1953125}{{(b) Relation-based Classification}}: Input a test image, the CLIP image encoder is adopted to extract the image feature. Next, the probability transposer is applied to convert the image classification probabilities from the prototypes to the target classes. This knowledge obtained from probability transformation is then incorporated with CLIP's pre-trained knowledge, achieving a training-free adaptation.
It should be noted that the "Tuned Parameters" in the figure refer only to the parameters that need to be fine-tuned in the training-required paradigm. However, these parameters can still contribute to improving CLIP's zero-shot performance even without fine-tuning.
}
\vspace{-4mm}
\label{fig:architecture}
\end{figure*}

The overall pipeline of our ICR-Transposer is shown in~\ref{fig:architecture}.
First, ICR-Transposer models the inter-class relation, and then obtains the classification logits using the probability transposer, introduced in~\ref{sec:arch}.
The Prototypes Prior Loss, which imposes constraints on the additional prototypes, further enhances the classification performance of CLIP, introduced in~\ref{sec:loss}.
The training and inference pipelines are illustrated in~\ref{train_and_infe}.

\subsection{Architecture}
\label{sec:arch}

Following~\cite{zhou2022learning}, we define the target classes prompts and the prototypes prompts given to the text encoder as follows:

\begin{equation}
    \boldsymbol{T}_{tgt,i}=[\boldsymbol{v}_1, \boldsymbol{v}_2, \boldsymbol{v}_3, ...,\boldsymbol{v}_M, \boldsymbol{s}_{tgt, i}]
    \label{eq:prompt_target}
\end{equation}

\begin{equation}
    \boldsymbol{T}_{pro,j}=[\boldsymbol{v}_1, \boldsymbol{v}_2, \boldsymbol{v}_3, ...,\boldsymbol{v}_M, \boldsymbol{s}_{pro, j}]
    \label{eq:prompt_auxiliary}
\end{equation}

where $i\in \{1, 2, ..., C_{tgt} \}$ is the target class index, $\boldsymbol{s}_{tgt, i}$ denotes word embedding of the $i$-th target class name $\mathrm{s}_{i}$, $j \in \{1, 2, ..., C_{pro} \}$ is the prototype index, the $\boldsymbol{s}_{pro, j}$ denotes word embedding of the $j$-th prototype name $\mathrm{s}_{j}$ if the propotype was designed manually else randomly initialized vector. For $k\in \{1, 2, ..., M\}$, $\boldsymbol{v}_{k}$ denotes word embedding of the $k$-th word of prompt sentences (\textit{e.g.} $\texttt{"A photo of \{\}."}$).

As shown in Fig.~\ref{fig:architecture}(a), by forwarding the target class prompts $\boldsymbol{T}_{tgt}$ and the prototypes prompts $\boldsymbol{T}_{pro}$ to the CLIP text encoder, we can obtain the target class features $\boldsymbol{F}_{tgt} \in \mathbb{R}^{C_{tgt} \times 
 D}$ and the prototype feature $\boldsymbol{F}_{pro} \in \mathbb{R}^{C_{pro} \times D}$. The features of target classes and prototypes are used to build the Inter-class Relation, the Inter-class Relation $\boldsymbol{R} \in \mathbb{R}^{ C_{tgt} \times C_{pro} }$ is defined as $\varphi(\boldsymbol{F}_{tgt} \boldsymbol{F}_{pro}^T)$:

% \begin{equation}
%      \boldsymbol{R}_{i,j} = \frac{\exp(\cos(
%      \boldsymbol{F}_{tgt, i},\boldsymbol{F}_{aux, j}
%      )/\tau)}{
% \sum\nolimits_{j=1}^{C_{aux}} \exp(\cos(
%      \boldsymbol{F}_{tgt, i},\boldsymbol{F}_{aux, j}
%      )/\tau) 
% } 
% \end{equation}

As shown in Fig.~\ref{fig:architecture}(b), by forwarding the test image $\boldsymbol{I} \in \mathbb{R} ^ {H \times W \times 3}$ to the CLIP image encoder, we can obtain the test image feature $f_{test} \in \mathbb{R} ^ {D}$.
The Probability Transposer is a cross-attention module, which accepts the image feature $f_{test}$ as query, the prototype features $\boldsymbol{F}_{pro}$ as keys, and the Inter-class Relation $\boldsymbol{R}$ as values. The processing of Probability Transposer is defined as:

\begin{equation}
    \rm{logits}_{ICR} = \texttt{CrossAttn}(f_{test}, \boldsymbol{F}_{aux}, \boldsymbol{R})
\end{equation}

% \begin{equation}
%     \rm{logits}_{ICR} = \texttt{CrossAttn}(f_{test}\boldsymbol{W}_{\rm{q}}^T, \boldsymbol{F}_{aux}\boldsymbol{W}_{\rm{k}}^T, \boldsymbol{R})
% \end{equation}

And the output logits are calculated as:

\begin{equation}
    \rm{logits} = \alpha \rm{logits}_{ICR} + f_{test} \boldsymbol{F}_{tgt}^T
\end{equation}


Probability Transposer's prediction, therefore, contains two terms, the former term is transformed by Inter-class Relation, and the latter term preserves the prior knowledge from the CLIP's classifier $\boldsymbol{F}_{tgt}$.

\subsection{Prototypes Prior Loss}
\label{sec:loss}

Based on the influence of manually selecting different prototypes on CLIP's zero-shot performance (which will be further investigated in the ablation study section~\ref{sec:ablation_on_auxiliary_selection}), we have identified the key characteristics that prototypes should possess to enhance CLIP's zero-shot performance:

$\bullet$ Prototypes should not exhibit an excessively high correlation with a single category in the target classes while having a very low correlation with other categories. In the extreme case where the prototype is identical to a target class, it does not contribute to improving CLIP's zero-shot performance. Therefore, any prototype should have associations with the target classes that significantly deviate from a one-hot distribution.

$\bullet$ Prototypes should not exhibit similar correlations with all categories in the target classes. In the extreme case where the prototype has identical similarities with all target classes, it also does not contribute to improving CLIP's zero-shot performance. Therefore, any prototype should have associations with the target classes that significantly deviate from a uniform distribution.

$\bullet$ There should not be target classes with extremely low correlations with any prototype. Such target classes would not benefit from the performance improvements derived from inter-class relations.

At first, we define the probability $\boldsymbol{P} \in \mathbb{R}^{ C_{tgt} \times C_{pro} }$ matrix as follows:

\begin{equation}
     \boldsymbol{P}_{i,j} = \frac{\exp(\cos(
     \boldsymbol{F}_{tgt, i},\boldsymbol{F}_{pro, j}
     )/\tau)}{
\sum\nolimits_{i=1}^{C_{tgt}} \exp(\cos(
     \boldsymbol{F}_{tgt, i},\boldsymbol{F}_{pro, j}
     )/\tau) 
} 
\end{equation}

In order to avoid the collapse of the probability distribution of $j$-th prototype belonging to target classes $\boldsymbol{P}_j = \{\boldsymbol{P}_{i,j}\}_{i=1}^{C_{tgt}}$ into a one-hot distribution, we can utilize k-means clustering to group the probability distribution into three clusters $\{\mathcal{C}\}_1^3$. Let $k$ represent the index of the cluster with the highest average value, as $ k = {\rm argmax}_{i} \{ \overline{\mathcal{C}_i} \}_1^3$. 
If the length of cluster $k$ is greater than $1$, the loss is assigned as 0. However, if the length of cluster $k$ is equal to $1$, we generate a probability pseudo-label $\boldsymbol{Q}_j = \{ 0.3\  \text{if}\  t\  \text{in}\  {\text{indices}_{top3}} \  \text{else}\  0.1 / (C_{tgt} - 3)\}_{1}^{C_{tgt}}$ and employ KL divergence as the loss function.

\begin{equation}
    \mathcal{L}_{KE} = 
    \begin{cases}
        0, & \text{if length of cluster } k > 1 \\
        \text{KL}(\boldsymbol{P}_j || \boldsymbol{Q}_j), & \text{if length of cluster } k = 1
    \end{cases} 
\end{equation}


To avert the similarity of the $j$-th auxiliary belonging to closes to a uniform distribution, we incorporate the entropy regularize, vis minimizing:

\begin{equation}
    \mathcal{L}_{EH} = \frac{ \sum -\boldsymbol{P}_j^T\log (\boldsymbol{P}_j) }{C_{pro}}
\end{equation}

To any target classes with extremely low correlations with any prototype, we incorporate the entropy regularize, vis minimizing:

\begin{equation}
    \mathcal{L}_{HE} =  \overline{\boldsymbol{P}_j}^T\log (\overline{\boldsymbol{P}_j}) 
\end{equation}


Finally, the Prototypes Prior Loss (PP loss) be defined as:

\begin{equation}
    \mathcal{L}_{PP} =  \mathcal{L}_{KE} + \mathcal{L}_{EH} + \mathcal{L}_{HE}
\end{equation}


\subsection{Training and Inference}
\label{train_and_infe}

\subsubsection{Zero-shot Setting}

We propose ZS-ICR-Transposer, an adaption method to enhance the zero-shot classification performance of CLIP. 
Our method introduces extra prototypes, which we distinguish from the target classes in the target domain. 
In a training-free manner, the zero-shot performance of CLIP is improved through the use of manually designed prototypes.
In a training-required manner, the zero-shot performance of CLIP can be enhanced by learning appropriate prototypes through random initialization and utilizing the Prototype Prior Loss in the ZS-ICR-Transposer framework.
In this manner, only the prototype embeddings are tuned, while the parameters of the probability transposer are frozen.

\subsubsection{Few-shot Setting}

ZS-ICR Transposer offers a substantial boost to CLIP by incorporating fresh inter-class relation knowledge, even without access to training data, and its performance can be further refined through optimization using the prior loss. 
Moreover, ICR-Transposer remains compatible with situations that involve training data. In the few-shot scenario, a limited amount of data can aid ICR-Transposer in acquiring superior auxiliary classes, thereby elevating its performance even further. 
ICR-Transposer focuses solely on updating the auxiliary class embeddings (which can be pre-designed or randomly initialized) to learn auxiliary classes that provide significant performance improvements to CLIP. 
With the updates made to ICR-Transposer, it attains state-of-the-art performance on 11 widely adopted datasets. For few-shot setting, we use the standard cross-attention transformer block as Probility Transposer.

The total loss be defined as:

\begin{equation}
    \mathcal{L} =  \mathcal{L}_{cls} + \gamma \mathcal{L}_{PP}
\end{equation}


==> section/Method-v2.tex <==
\section{Method}
\label{method}

\begin{figure*}
\begin{center}
\includegraphics[width=1.0\linewidth]{figure/architecture.pdf}
\end{center}
   \vspace{-3mm}
\caption{\textbf{The Pipeline of \textcolor{blue}{Our Method}.} 
\textcolor[rgb]{0.796875, 0.3984375, 0.0}{{(a) Anchor-target Relation Modelling}}: Input with target categories and anchors, CLIP text encoder is adopted to extract target features $\mathcal{F}_{tar}$ and anchor features $\mathcal{F}_{pro}$, which are used to model anchor-target relation matrix $\mathcal{R}$ between target categories and anchors. 
% Where the anchor classes can either be randomly initialized or designed manually.
\textcolor[rgb]{0.35546875, 0.5546875, 0.1953125}{{(b) Relation Transition}}: Input a test image $\mathcal{I}$, CLIP image encoder is adopted to extract the image visual feature. Next, the Relation Transition Module (RTM) $\Phi$ is applied to transition image-anchor relation to image-target relation. CLIP classifier is initialized using target features $\mathcal{F}_{tar}$. The knowledge acquired from relation transition is then integrated with CLIP's pre-trained knowledge, enabling accurate prediction.
% It should be noted that the "Tuned Parameters" in the figure refer only to the parameters that need to be fine-tuned in the training-required paradigm. However, these parameters can still contribute to improving CLIP's zero-shot performance even without fine-tuning.
}
\vspace{-4mm}
\label{fig:architecture}
\end{figure*}

The overall pipeline of \textcolor{blue}{our method} is shown in Fig.~\ref{fig:architecture}.
%how to get anchor class?
Given target categories and anchors, we first construct the anchor-target relation matrix to model the anchor-target relationship between them, where anchors can be either initialized by cross-dataset category list or randomly initialized, introduced in Sec.~\ref{sec:icr_model}.
The image visual feature extracted by CLIP image encoder, anchors features, and anchor-target relation matrix are used as queries, keys, and values of the relation transition module (\textbf{RTM}) to 
convert the image-anchor relations to image-target relations, achieving relation transition. 
Then, the relation-based classification works in conjunction with CLIP's zero-shot classifier to produce the final prediction, described in Sec.~\ref{relation_based_cls}.
The training and inference pipelines are illustrated in Sec.~\ref{train_and_inference}.




\subsection{Anchor-target Relation Modelling}
\label{sec:icr_model}

% 1. target categories 是什么
% 2. 我们提出了一些 anchors (为什么提出)
% 3. 变量的尺寸, D = 512, D 是什么东西

% 1. target categories 是什么
In this paper, our primary task focuses on zero-shot and few-shot image classification, where we aim to classify images into their respective categories with limited or no training examples available for the target categories. 
The target categories serve as a set of labels for the classification task. 
% However, the aligned CLIP image/text encoders contain abundant relationships between visual features and almost infinite open semantics, 
% which may benefit the few-shot learning but remains unexplored. 
% In this paper, we focus on mining open semantics as anchors to perform a relation transition from 
% image-anchor relationship to image-target relationship to make predictions.
Our primary goal is to mine these open semantics to improve the CLIP's classification performance.
We use anchors as cues derived from the open semantics within CLIP. 
Anchors serve as a bridge to connect and transition image features to their corresponding target categories in image classification task.
To be more specific, anchors can take different forms depending on their origin and semantics. 
For instance, anchors can be category names sampled from cross-dataset category list, which carry explicit semantic information. 
Alternatively, they may be randomly initialized class tokens that do not hold any clear semantic information.
We model the anchor-target relation, which is used to transition the image-anchor relation to image-target relation.

The anchor-target relation is modeled using the CLIP text encoder.
Following~\cite{zhou2022learning}, we define the target categories prompts $\mathcal{T}_{tar}$ and the anchors prompts $\mathcal{T}_{anc}$ given to the text encoder as follows:

\begin{align}
\mathcal{T}_{tar,i}\;&=[\boldsymbol{v}_1, \boldsymbol{v}_2, ...,\boldsymbol{v}_M, \boldsymbol{s}_{tar, i}\;] \\
\mathcal{T}_{anc,j}&=[\boldsymbol{v}_1, \boldsymbol{v}_2, ...,\boldsymbol{v}_M, \boldsymbol{s}_{anc, j}]
\end{align}

where $i\in \{1, 2, ..., C_{tar} \}$ is the target categories index, $C_{tar}$ denotes the number of target categories, $\boldsymbol{s}_{tar, i}$ denotes word embedding of the $i$-th target categories name $\mathrm{s}_{i}$,
$j \in \{1, 2, ..., C_{anc} \}$ is the anchors index, $C_{anc}$ denotes the number of anchors, the $\boldsymbol{s}_{anc, j}$ denotes word embedding of the $j$-th anchors name $\mathrm{s}_{j}$.
The anchors are initialized by cross-dataset category list or randomly initialized in the experiments. 
$[\boldsymbol{v}_1, \boldsymbol{v}_2, ...,\boldsymbol{v}_M]$ denotes word embedding of the prompt sentences prefix (\textit{e.g.} $\texttt{"A photo of \{\}."}$).

After obtaining the text feature, as shown in Fig.~\ref{fig:architecture}(a), by forwarding the target categories prompts $\mathcal{T}_{tar}$ and the anchors prompts $\mathcal{T}_{anc}$ to the CLIP text encoder, we can obtain the target L2 normalized features $\mathcal{F}_{tar} \in \mathbb{R}^{C_{tar} \times D}$ and the anchor L2 normalized features $\mathcal{F}_{anc} \in \mathbb{R}^{C_{anc} \times D}$. 
Where $D$ denotes the feature dimension of the CLIP's visual-language feature space
(\textit{e.g.} $D=512$ for ResNet50~\cite{he2016deep} backbone in CLIP). 
% For instance, the feature dimension $D$ is 512 when the CLIP's image backbone is ResNet50~\cite{he2016deep}.
The features of target categories and anchors are used to build anchor-target relation matrix $\mathcal{R} \in \mathbb{R}^{ C_{tar} \times C_{anc} }$ to model the anchor-target relation. 
The anchor-target relation matrix $\mathcal{R}$ is defined in Equation.~\ref{cls_shift_matrix}.

\begin{equation}
     \mathcal{R}_{i,j} = \frac{\exp(\cos( \mathcal{F}_{tar, i},\mathcal{F}_{anc, j} )/\tau)}{
\sum\nolimits_{j=1}^{C_{anc}} \exp(\cos( \mathcal{F}_{tar, i},\mathcal{F}_{anc, j} )/\tau) 
} 
\label{cls_shift_matrix}
\end{equation}

\subsection{Relation Transition}
\label{relation_based_cls}

% 
% 首先讲 Zero-shot
% 之后讲，人为设计的逻辑不一定是好的，有数据之后，就可以用Transformer构建更好的关系

As shown in Fig.~\ref{fig:architecture}(b), by forwarding the test image $\mathcal{I} \in \mathbb{R} ^ {H \times W \times 3}$ to the CLIP image encoder, we can obtain the test image L2 normalized feature $f_{test} \in \mathbb{R} ^ {D}$.
The Relation Transition Module (RTM) $\Phi$ is a cross-attention module, which accepts the image visual feature $f_{test}$ as "Query", anchor features $\mathcal{F}_{anc}$ as "Key", and the anchor-target relation matrix $\mathcal{R}$ as "Value" to transition image-anchor relation to image-target relation, defined as $\mathcal{P}_{tar} = \Phi (f_{test}, \mathcal{F}_{anc}, \mathcal{R})$. 

For the zero-shot setting, the image-anchor relation $\mathcal{P}_{anc} \in \mathbb{R} ^ {C_{anc}}$ is calculated as

\begin{equation}
    \mathcal{P}_{anc,j} = \frac{
    \exp( \cos(f_{test}, \mathcal{F}_{anc,j}) / \tau )
    }{
    \sum_{j=1}^{C_{anc}} \exp( \cos(f_{test}, \mathcal{F}_{anc,j}) / \tau )
    } .
\end{equation}

% Then, the image classification probabilities from the anchor classes $\mathcal{P}_{anc}$ to the probabilities of target classes $\mathcal{P}_{tar}$ through
Then, the Relation Transition Module (RTM) performs a relation transition from  image-anchor relation $\mathcal{P}_{anc}$ to image-target relation $\mathcal{P}_{tar}$. This transition is defined as 

\begin{equation}
    \mathcal{P}_{tar,i} = \frac{
    \exp( \cos(\mathcal{P}, \mathcal{R}_{i}) / \tau' )
    }{
    \sum_{i=1}^{C_{tar}} \exp( \cos(\mathcal{P}, \mathcal{R}_{i}) / \tau' )
    } .
\end{equation}

For the few-shot setting, we use the transformer architecture as RTM $\Phi$. The image-target relation is obtained by

\begin{equation}
    \mathcal{P}_{tar} = \text{Transformer} (f_{test}, \mathcal{F}_{anc}, \mathcal{R}).
\end{equation}

Then, the relation-based prediction $\mathcal{P}_{tar}$ works in conjunction with CLIP's zero-shot prediction $\mathcal{P}_{clip}$ to produce the final prediction $\mathcal{P}_{final}$.


\begin{equation}
    \mathcal{P}_{final} = \mathcal{P}_{clip} + \alpha \mathcal{P}_{tar}
\end{equation}


In this way, we mine open semantics as anchors to perform a relation transition from 
image-anchor relation to image-target relation.

\subsection{Training and Inference}
\label{train_and_inference}

\textbf{Zero-shot Setting.}
In the zero-shot setting, our method does not require any training, and we refer to it as ZS-ICR-Transposer.
% First, we manually design the anchor categories according to the target categories. 
% initialized by cross-dataset category list
First, we manually select anchors from cross-dataset category list. 
Then, we build the anchor-target relation matrix $\mathcal{R}$ to model anchor-target relationship. 
The anchor-target relation matrix only needs to be created once, which means that we only need to perform one forward pass of the CLIP text encoder. Once the anchor-target relation is established, the CLIP text encoder can be discarded.
Next, the Relation Transition Module $\Phi$ is applied to convert the image-anchor relation $\mathcal{P}_{anc}$ to the image-target relation $\mathcal{P}_{tar}$. 
Finally, the relation-based prediction $\mathcal{P}_{tar}$ collaborates with CLIP's zero-shot prediction $\mathcal{P}_{zs}$ to produce the final prediction $\mathcal{P}_{final}$.

% We propose ZS-ICR-Transposer, an adaption method to enhance the zero-shot classification performance of CLIP. 
% Our method introduces extra anchor categories, which we distinguish from the target classes in the target domain. 
% In a training-free manner, the zero-shot performance of CLIP is improved through the use of manually designed prototypes.
% In a training-required manner, the zero-shot performance of CLIP can be enhanced by learning appropriate prototypes through random initialization and utilizing the Prototype Prior Loss in the ZS-ICR-Transposer framework.
% In this manner, only the prototype embeddings are tuned, while the parameters of the probability transposer are frozen.

\textbf{Few-shot Setting.}
\textcolor{blue}{ZS-ICR-Transposer} offers a substantial boost to CLIP by incorporating fresh open semantics relation transition knowledge. 
Moreover, \textcolor{blue}{ICR-Transposer} remains compatible with situations that involve training data. 
In the few-shot scenario, a limited amount of data can aid \textcolor{blue}{ICR-Transposer} in acquiring superior anchors, thereby elevating its performance even further. 
\textcolor{blue}{ICR-Transposer} focuses solely on updating the anchors embeddings (which can be pre-designed or randomly initialized) to learn anchor classes that provide significant performance improvements to CLIP. 
For few-shot setting, we use cross entropy loss to update ICR-Transposer.
With the updates made to \textcolor{blue}{ICR-Transposer}, it attains state-of-the-art performance on 11 widely adopted datasets. 


==> section/RelatedWork-v0.tex <==
\section{Related Work}

\subsection{Multimodel Foundation Models}

Recently, foundation models have shifted towards a multimodel supervision paradigm. 
CLIP~\cite{radford2021learning} and ALIGN~\cite{jia2021scaling} propose a simple contrastive-based approach to embed images and texts into the same representation space, and demonstrate impressive "zero-shot" performance on downstream tasks.
FILIP~\cite{yao2021filip} captures fine-grained semantic relationships between images and text in dual-encoder methods for image-text matching by using a token-wise maximum similarity approach.
LOUPE~\cite{li2022fine} explicitly learns the fine-grained semantic alignment between visual regions and textual phrases through Shapley value.
UniCLIP~\cite{lee2022uniclip} improves data efficiency by integrating contrastive losses defined across multiple domains into a single universal space.
PyramidCLIP~\cite{gao2022pyramidclip} constructs an input pyramid with different semantic levels for each modality.
In this work, we focus on adapting CLIP~\cite{radford2021learning} for zero-shot and few-shot classification.


\subsection{Data-efficient Transfer Learning}


Deep neural networks have demonstrated impressive capabilities in various tasks, but they heavily rely on large-scale and high-quality datasets~\cite{deng2009imagenet,gupta2019lvis}. 
Unfortunately, collecting such data can be challenging and expensive, mainly due to factors such as long-tail distributions, noisy annotations, and increasing labeling costs. 
As a solution, transfer learning has emerged as a popular research field to address these issues. 
Transfer learning involves utilizing pre-trained models on large datasets to enhance the learning of new models on smaller datasets. 
Vision-language models have demonstrated their zero-shot recognition capability across diverse datasets. 
Recent approaches adopt the prompt-based paradigm~\cite{zhou2022learning,zhou2022conditional,zhu2022prompt,lu2022prompt,sun2022dualcoop} and adapter-based paradigm~\cite{gao2021clip,zhang2022tip} instead of fine-tuning the entire model~\cite{dong2022clip}, as fine-tuning may damage the learned representation space.

We adopt the training-free paradigm of Tip-Adapter~\cite{zhang2022tip}, which infuses few-shot supervisions into the pre-trained CLIP model. However, in contrast to Tip-Adapter, we directly use the CLIP Text Encoder to construct an Inter-class Relation and infuse it into the CLIP model. Importantly, our approach does not require any additional data compared to Tip-Adapter. 
In comparison to the prompt-based paradigm, our method differs in that we finetune class embeddings rather than prompt embeddings.

==> section/RelatedWork-v1.tex <==
\section{Related Work}

\subsection{Adaptation of Vision-Language Pre-trained Models}

Recently, there has been a growing trend in AI towards the dominant paradigm of learning foundation models~\cite{bommasani2021opportunities} from large-scale web data.
The development of Vision-Language Pre-trained Models~\cite{radford2021learning,jia2021scaling,yao2021filip,li2022fine,lee2022uniclip,gao2022pyramidclip,zhou2022non} has been particularly rapid, thanks to the low cost of collecting image-text pairs from the web. 
In this work, we focus on adapting CLIP~\cite{radford2021learning} for zero-shot and few-shot classification. 
With the remarkable performance of multimodal pre-trained models in classic vision tasks~\cite{radford2021learning,zhang2022glipv2}, there has been a surge of interest in the development of more efficient adaptation methods. 
However, it is worth noting that while many trending techniques concentrate on extracting and utilizing features from CLIP, the exploration of leveraging these semantic associations to enhance CLIP's performance in downstream tasks remains largely unexplored.
For instance, when transferring to downstream tasks, CLIP commonly employs linear probing~\cite{chen2020simple,he2022masked} and full-finetuning~\cite{girdhar2017attentional,dong2022clip} techniques.
Prompt tuning of CLIP~\cite{radford2021learning,zhou2022conditional,lu2022prompt,xing2022class,zhu2022prompt,sun2022dualcoop} draws inspiration from the successful implementation of prefix-tuning in language models~\cite{deng2022rlprompt,gao2020making,haviv2021bertese,jiang2020can}, specifically aiming to extract broader text features.
Similarly, CLIP-Adapter~\cite{gao2021clip} and Tip-Adapter~\cite{zhang2022tip} draw inspiration from parameter-efficient fine-tuning methods~\cite{houlsby2019parameter,jia2022visual,zhang2020side} that optimize lightweight MLPs while keeping the encoder frozen. 
These approaches leverage features from CLIP to enhance performance. 
Our focus lies in exploring the untapped potential of leveraging the semantic associations constructed by CLIP.


\subsection{Few-shot Classification}

Previous successful methods for few-shot learning have utilized techniques such as meta-learning~\cite{finn2017model,ravi2017optimization}, metric learning~\cite{bateni2020improved,snell2017prototypical,vinyals2016matching,sung2018learning}, transfer learning~\cite{hariharan2017low,qi2018low}, and transductive learning~\cite{dhillon2019baseline,joachims1999transductive}.
Instead of following the traditional approach of evaluating on multiple few-shot train and test sets, we adopt a new evaluation protocol implemented by recent works on few-shot adaptation with CLIP~\cite{radford2021learning}. 
In this protocol, we replace the meta-training phase with pre-trained CLIP models, and the test sets used are the official test splits of each dataset. 


\subsection{Relationship-based Approaches}

In the field of NLP, HRKD~\cite{dong2021hrkd} enhances model capability and transferability by establishing domain-relational graphs that capture relational information across diverse domains.
In the field of CV, Co-tuning~\cite{you2020co} leverages training samples to learn the relationship between source domain categories and target domain categories from a pre-trained model, aiding in the learning of the target domain classification head. 
Co-tuning establishes associations between categories to some extent, but these category associations are based on target domain training samples, which can introduce biases, especially in data-limited scenarios.
Our approach effectively leverages the semantic associations constructed by CLIP and utilizes them to significantly improve the classification performance of CLIP.

==> section/temporary.tex <==



Model Name:              ?
Auxiliary Class Name:    anchors
Inter-class Relation:    anchor-target relation matrix
Prob. Transposer:        relation transition module (RTM)
Rule1:                   A reasonable prior is that the image-target relations should keep consistent after relation transition, no matter whether relation transition is performed.


Through the transition of anchor-target relation matrix, the image-target relations can be obtained. 
A reasonable prior is that the image-target relations should keep consistent after relation transition, 
\emph{e.g.}, an image of "chinchilla" should be classified into the "chinchilla" category, no matter whether relation transition is performed.

we design the relation transition module (RTM) as a transformer 
decoder architecture which takes the visual feature as "Query",
the text features of the anchors as "Key" and the similarity matrix between the text features of 
anchors and target classes as "Value".




























URVOS overleaf: https://www.overleaf.com/6172521637rjzmmshkzryx

ICR code: https://anonymous.4open.science/r/ICR-Transposer


% ?
Model Name:              ICR-Transposer
Auxiliary Class Name:    Anchor Categories
Inter-class Relation:    class-shifting matrix
Loss:                    Anchor Loss


Background & Problem?
Previous Model:
1. using data? % 感觉这个点太小?
2. focused on extracting and utilizing features from CLIP to enhance performance % 感觉概括的不太准, 也不太好过度到 Relation?


Intro
Contribution
1. semantic -> model 想法
2. 具体实现
3. SOTA


zero-shot - 语义关联 cross model

related work
1. traditional few-shot learning
2. CLIP-based few-shot learning
3. zero-shot 相关论文 (optional) 


图:

prompt -> A photo of {}
class 前面 加 e.g.
Prob. Transposer -> Transformer
CLIP Classifier 在 caption 说用什么初始化

Ablation
行 softmax 如果有用（看增益）：
行 softmax + 列 softmax (ensemble) 
如果没用：
行 softmax + 列 softmax 在实验方法写


1. Zero-shot (前三行), Random Init.|2 和 Classes Init.|3 对比作为引子
2. heatmap learnable 的 feature 和 classes init.
3. Table4. 把 rand 和 class embed 改成 ours, 在 caption 说
4. Tip-Adap 方式 和 transformer 方式对比
